Many Hands Make Light Work: Accelerating Edge Inference via Multi-Client Collaborative Caching

Edge inference is a technology that enables real-time data processing and analysis on clients near the data source. To ensure compliance with the Service-Level Objectives (SLOs), such as a 30% latency reduction target, caching is usually adopted to reduce redundant computations in inference tasks on stream data. Due to task and data correlations, sharing cache information among clients can improve the inference performance. However, the non-independent and identically distributed (non-IID) nature of data across different clients and the long-tail distributions, where some classes have significantly more samples than others, will reduce cache hit ratios and increase latency. To address the aforementioned challenges, we propose an efficient inference framework, CoCa, which leverages a multi-client collaborative caching mechanism to accelerate edge inference. On the client side, the model is pre-set with multiple cache layers to achieve a quick inference. During inference, the model performs sequential lookups at cache layers activated by the edge server. On the server side, CoCa uses a two-dimensional global cache to periodically aggregate information from clients, mitigating the effects of non-IID data. For client cache allocation, CoCa first evaluates the importance of classes based on how frequently and recently their samples have been accessed. CoCa then selects frequently recurring classes to address long-tail distribution challenges. Finally, CoCa dynamically activates cache layers to balance lookup overhead and accuracy. Extensive experiments demonstrate that CoCa reduces inference latency by 23.0% to 45.2% on the VGG, ResNet and AST models with a slight loss of accuracy.

==> content/analysis.tex <==
In this section, we provide the convergence analysis of the proposed framework.
We first state the following assumptions, which are standard in non-convex optimization problems (\eg, training deep neural networks) and are widely used in the analysis of previous works \cite{jiang2023computation}.

\noindent\textbf{Assumption 1.} \textbf{(\textit{Smoothness})} The local objective function $F_{n}$ of each client $n$ is smooth with modulus $L$:
% \vspace{1mm}
\begin{equation}
    F_{n}(\mathbf{y}) - F_{n}(\mathbf{x}) \leq \frac{L}{2} \| \mathbf{y} - \mathbf{x} \|^{2} + \langle \nabla F_n(\mathbf{y}), \mathbf{y} - \mathbf{x} \rangle \quad \forall n, \mathbf{x}, \mathbf{y} 
\end{equation}
\vspace{0.1mm}
\noindent\textbf{Assumption 2.} \textbf{(\textit{Bounded Variance})} 
Let $\xi_{n}$ denote a random data batch sampled from client $n$'s local dataset $D_{n}$. 
% Let $D_{n}$ denote the local dataset of client $n$ and $\xi_{n}$ is a data batch randomly sampled from $D_{n}$.
There exists a constant $\sigma > 0$ such that the variance of stochastic gradients at each client is bounded by:
\begin{equation}
    \mathbb{E} [ \| \nabla F_{n}(\mathbf{x}; \xi_{n}) - \nabla F_{n} (\mathbf{x}) \|^{2} ] \leq \sigma^{2} \quad \forall \mathbf{x}, n, \xi_{n} 
\end{equation}
\vspace{0.1mm}
\noindent\textbf{Assumption 3.} \textbf{(\textit{Bounded Gradients})} There exists a constant $G>0$ such that the stochastic gradients at each client are bounded by:
\begin{equation}
    \mathbb{E} [ \| \nabla F_{n}(\mathbf{x}; \xi_{n}) \|^{2} ] \leq G^{2} \quad \forall \mathbf{x}, n, \xi_{n}  
\end{equation}
% For the convenience of analysis, we assume that all clients participate in training at each round (\ie, $K=N$). 
% For the convenience of analysis, we use the element-wise product to represent coefficients at different width.
For the convenience of analysis, we represent the reduced coefficient by an element-wise product, \ie, $\hat{\mathbf{u}}^{h}_{n} = \mathbf{u}^{h} \odot \mathbf{m}^{h}_{n}$, where $\mathbf{u}^{h}$ is the global coefficient in round $h$ and $\mathbf{m}^{h}_{n}$ is the corresponding binary mask for client $n$ in round $h$. 
Physically, the masked blocks are removed from the coefficient and the remaining blocks are composited with basis to the local model $\hat{\mathbf{x}}^{h}_{n}$, which can be denoted as $\mathbf{v}^{h} \cdot (\mathbf{u}^{h} \odot \mathbf{m}^{h}_{n})$. 
% To express the error induced by pruning coefficient, we adopt an upper bound $\beta^{2}$, where $\| \mathbf{u}^{h} - \hat{\mathbf{u}}^{h}_{n} \|^{2} \leq \beta^{2}$.
After the neural composition, each client $n$ sets $\hat{\mathbf{x}}^{h}_{n} (0) = \hat{\mathbf{x}}^{h}_{n}$ and performs $\tau^{h}_{n}$ local iterations by mini-batch SGD optimizer over its local dataset $D_{n}$.
Specifically, at each local iteration $t \in \{1, 2, \cdots, \tau^{h}_{n} \}$, the local model can updated as follows:
\begin{equation}
    \hat{\mathbf{x}}^{h}_{n}(t) = \hat{\mathbf{x}}^{h}_{n}(t-1) - \eta \nabla F_{n}(\hat{\mathbf{x}}^{h}_{n}(t-1); \xi_{n}) \odot \mathbf{m}_{n}^{h}
\end{equation}
where $\eta$ is the learning rate. In order to analyse the convergence bound of the global loss function after $H$ rounds, we present the following three important lemmas.

\noindent\textbf{Lemma 1.} According to Assumption 3, the deviations between global model $\mathbf{x}^{h}$ and local model $\hat{\mathbf{x}}^{h}_{n}(t-1)$ can be bounded as:
\begin{align}
    & \! \! \! \! \! \! \sum_{t=1}^{\tau} \sum_{n=1}^{N} \mathbb{E} [\| \mathbf{x}^{h} - \hat{\mathbf{x}}_{n}^{h}(t - 1) \|^{2} ] \leq \frac{2 \tau^{3} \eta^{2} G^{2} N }{3} + 2 \tau \sum_{n=1}^{N} \alpha_{n}^{h} 
\end{align}
where $\alpha_{n}^{h}$ represents the model error induced by reducing coefficient (\ie, $ \alpha_{n}^{h} \triangleq  \|\mathbf{u}^{h} - \hat{\mathbf{u}}^{h}_{n} \|^{2}$) and $\tau = \mathop{\max} \{ \tau_{n}^{h} \}$.
 
\noindent\textbf{Lemma 2.} Combining Assumptions 1-2 and Lemma 1, the difference between global models in two successive rounds can be bounded as:
\begin{align}
    &  \mathbb{E} [\| \mathbf{x}^{h+1} - \mathbf{x}^{h} \|^{2}] \leq  3 \eta^{2} \tau^{2} \mathbb{E} [\|  \nabla F_{n} (\mathbf{x}^{h})  \|^{2}]  \notag \\
    & +  \frac{6 \eta^{2} \tau^{2} L^{2}}{N} \sum_{n=1}^{N} \alpha_{n}^{h} + 2 \tau^{4} \eta^{4} G^{2} L^{2} + 3 \eta^{2} \tau^{2} \sigma^{2} \label{eq:lemma_2}
\end{align}

\noindent\textbf{Lemma 3.} Under Assumption 1 and Lemma 1, the proposed framework ensures:
\begin{align}
    &\mathbb{E}[\langle \nabla F(\mathbf{x}^{h}), \mathbf{x}^{h+1} - \mathbf{x}^{h} \rangle ]  \notag \\
    \leq & - \frac{\tau \eta}{2} \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] + \frac{L^{2} \tau \eta}{N} \sum_{n=1}^{N} \alpha_{n}^{h} + \frac{\tau^{3} \eta^{3} L^{2} G^{2}}{3} \label{eq:lemma_3}
\end{align}

Let these assumptions and lemmas hold, we obtain the convergence bound as shown in Theorem 1.

\noindent\textbf{Theorem 1.} If the learning rate satisfies $\eta \leq \frac{1}{6L\tau}$, the mean square gradient after $H$ rounds can be bounded as follows:

\begin{align}
    & \frac{1}{H} \sum_{h=0}^{H-1} \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] \leq \frac{4}{H \eta \tau} (F(\mathbf{x}^{0}) - F(\mathbf{x}^{*})) \notag \\
    &  + \frac{6 L^{2}}{H N} \sum_{h=0}^{H-1} \sum_{n=1}^{N} \alpha_{n}^{h} + \frac{L \eta \tau }{3} ( G^{2} + 18 \sigma^{2} ) \label{eq:theorem_1}
\end{align}
where $\mathbf{x}^{*}$ denotes the optimal global model. 

\noindent\textit{Proof. } With the smoothness assumption, we have:

\begin{align}
    & \mathbb{E}[F(\mathbf{x}^{h+1})] - \mathbb{E}[F(\mathbf{x}^{h})] \notag \\
    \leq & \frac{L}{2} \mathbb{E} [\| \mathbf{x}^{h+1} - \mathbf{x}^{h} \|^{2}] + \mathbb{E}[\langle \nabla F(\mathbf{x}^{h}), \mathbf{x}^{h+1} - \mathbf{x}^{h} \rangle ] \label{eq:theorem_1_smooth} \\ 
    \leq & \frac{\tau \eta}{2}(3 \tau \eta L - 1) \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] + \frac{L^{2}\tau\eta}{N}(3 L \tau \eta + 1) \sum_{n=1}^{N} \alpha_{n}^{k} \notag \\
    & + \tau^{4} \eta^{4} L^{3} G^{2} + \frac{3 \eta^{2} \tau^{2} \sigma^{2} L}{2} + \frac{\tau^{3} \eta^{3} L^{2} G^{2}}{3} \label{eq:theorem_1_taking_lemmas_2_3}
\end{align}
where Eq. \eqref{eq:theorem_1_taking_lemmas_2_3} is obtained by taking Eq. \eqref{eq:lemma_2} and Eq. \eqref{eq:lemma_3} into Eq. \eqref{eq:theorem_1_smooth}. Summing over the round $h \in \{0, 1, \cdots, H-1 \}$ on the both sides of Eq. \eqref{eq:theorem_1_taking_lemmas_2_3}, we have:

\begin{flalign}
    & \mathbb{E}[F(\mathbf{x}^{H})] - \mathbb{E}[F(\mathbf{x}^{0})] \leq \tau^{4} \eta^{4} L^{3} G^{2} K  \notag \\
    & + \frac{\tau \eta}{2}(3 \tau \eta L - 1) \sum_{h=0}^{H-1} \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] + \frac{3 \eta^{2} \tau^{2} \sigma^{2} K L}{2} \notag \\
    & + \frac{L^{2}\tau\eta}{N}(3 L \tau \eta + 1) \sum_{h=0}^{H-1} \sum_{n=1}^{N} \alpha_{n}^{k} + \frac{\tau^{3} \eta^{3} L^{2} G^{2} K}{3} \label{eq:theorem_1_sum}
\end{flalign}
When the learning rate satisfies $\eta \leq \frac{1}{6L\tau}$, we can shift the terms in Eq. \eqref{eq:theorem_1_sum} as follows:

\begin{align}
    & \frac{\tau \eta}{4} \sum_{k=0}^{H-1} \mathbb{E}[\| \nabla F(\mathbf{x}^{h}) \|^{2}] \leq \mathbb{E}[F(\mathbf{x}^{0})] - \mathbb{E}[F(\mathbf{x}^{H})] \notag \\
    & + \frac{3 L^{2} \tau \eta}{2 N} \sum_{h=0}^{H-1} \sum_{n=1}^{N} \alpha_{n}^{h} + \frac{\tau^{2} \eta^{2} H L}{12} ( G^{2} + 18 \sigma^{2} ) \label{eq:theorem_1_shift}
\end{align}

Finally, we divide both sides of Eq. \eqref{eq:theorem_1_shift} by $\frac{H \eta \tau}{4}$ to derive the convergence bound in Eq. \eqref{eq:theorem_1} of Theorem 1.

Thus, we complete the convergence analysis of the proposed framework under non-convex setting.
The convergence bound is proportional to the coefficient reducing error. 
The larger the coefficient $\mathbf{u}_{n}^{h}$, the smaller the reducing error $\alpha_{n}^{h}$, leading to a tighter convergence bound.
Besides, the bound also depends on the local updating frequency, indicating that we can obtain better convergence performance by setting the local update frequency $\tau$ properly.








 

==> content/framework9.tex <==
\subsection{System Overview}
Inspired by the above observations, we introduce CoCa, an efficient inference framework with a multi-client collaborative caching mechanism. 
The workflow of CoCa is illustrated in Fig. \ref{fig:overview}. 
% 
The server first deploys pre-trained models to each client. Then, it iteratively performs the following steps round-by-round.
% 
At the beginning of each round, each client uploads its status information of the current data class distribution , such as timestamp vectors, to the server. 
Next, the server allocates the appropriate cache to each client based on the global commonality information and the status information of the client. 
The client then loads the received cache and performs local inference on some frames, during which it collects status information of clients and semantic vectors of inference samples. 
% 
At the end of the round, each client uploads the information collected in the current round to the server for global updates, such as updating the global cache table and class frequency information, and then prepares for the next round.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{fig/CoCa_Flow2.pdf}
  \caption{\textcolor{blue}{Overview of CoCa.} }
  \label{fig:overview}
\end{figure}



\subsection{Local Inference and Information Collection}
% 参数 和等式格式 待统一
On the client side, CoCa primarily involves the collection of status information of clients and semantic vectors of inference samples during local inferences. 
%(Lines \ref{4}-\ref{16} of Algorithm \ref{alg:CoCa}). 
At the beginning of CoCa, the client initializes two one-dimensional vectors to track the recent occurrences of data classes: a timestamp vector $\bm{\tau}$ and a local class frequency vector $\bm{\varphi}$.
Specifically,
we use ${\tau}_{i}$ (the $i$-th element of $\bm{\tau}$) to represent the number of inference processes since the last appearance of a sample of class $i$. After each inference process, the timestamp of the current sample class is reset to zero, while the timestamps of other classes are incremented by one.
We use ${\varphi}_{i}$ (the $i$-th element of $\bm{\varphi}$) to record the number of times that samples of class $i$ have appeared within the current round.
These vectors enable the client to maintain a dynamic record of recent class occurrences.
CoCa operates in rounds, processing $F$ frames in each round. Based on our tests, we set $F = 300$ to achieve stable periodic cache updates and uploads of client information.
% 
During local inference, the client maintains status information $\bm{\tau}, \bm{\varphi}$ and collects the cache update table $\mathbf{U}$ for global updates.
The cache update table has the same dimensions as the global cache table on the server. 
The client determines whether to collect information from the current inference process to populate $\mathbf{U}$ based on the following strategy.
Specifically, two types of inference samples will be chosen:
\begin{enumerate}
    \item Samples where the cache hits and the discriminative score ${D}_j$ (hits at the cache layer $j$) exceeds the threshold ${\Gamma}$. 
    These samples exhibit similar features to the current cache and can be used to reinforce it, thereby capturing the gradual evolution of class semantics over time. The collected semantic vectors are limited to the point of the cache hit.

    \item Samples where the cache misses and their normalized probability vectors $\mathbf{prob}$ of classes satisfy the following condition: the difference between the two largest probabilities, \ie, ${prob}_1 - {prob}_2$, is greater than the threshold ${\Delta}$. These samples display high confidence in the classification results but may not be adequately captured by the current cache, serving as a supplement to the global cache.
\end{enumerate}
These two types of samples represent the reinforcement and expansion of the current cache entries, respectively. The balance between reinforcement and expansion can be adjusted by tuning the two thresholds ${\Gamma}$ and ${\Delta}$.

% \begin{algorithm}[t]
% 	\caption{ Procedure of CoCa } \label{alg:CoCa}
%   \SetAlgoNoEnd
%     \SetAlgoNoLine
% 	\begin{algorithmic}[1]
%         \State \textbf{Client side}:
%         \State Initialize DNN model with total $L$ cache layers, local timestamp vector $\bm{\tau}$ and local class frequency vector $\bm{\varphi}$.
%         \While {True}
%             \State Upload $\bm{\tau}$ and request cache.\label{4}
%             \State Initialize the cache update table $\mathbf{U}$.
%             \For{ $i=1$ to $F$ }
%                 \For{ $j=1$ to $L+1$ } 
%                     % \Statex \Comment{$L$ is the number of all cache layers}
%                     \State Process frame $i$ through model block $j$
%                     \If{cache layer $j$ available}
%                         \State Extract the semantic vector $\mathbf{V}_j$.
%                         \State Perform cache lookups.
%                         \If{ cache hits }
%                             \State Exit early.
%                 \State Update $\bm{\tau}$, $\bm{\varphi}$.
%                 \State Update $\mathbf{U}$ by Eq. (\ref{eq:update U}).
%             \State Upload $\mathbf{U}$ and $\bm{\varphi}$ for the global updates. \label{16}
%         % server
%         \State \textbf{Server side}: 
%         \State Initialize the DNN model, global class frequency vector $\bm{\Phi}$, and global cache table $\mathbf{E}$. 
%         \State Let $\mathcal{K} = \{1, 2, ..., N\}$ be the set of all clients
%         \While {True}
%             \For {each client  $k \in \mathcal{K}$ (in parallel)}
%                 \State Receive cache allocation request from client $k$, along with decision-support information, such as $\bm{\tau}^k$. \label{19}
%                 %\State  cache entry by Algorithm \ref{alg:cache select}.
%                 \State Allocate the proper cache to client $k$ by Alg. \ref{alg:cache select}.  \label{21}
%                 \State Wait for client $k$ to complete local inference
%                 \State Receive $\mathbf{U}^k$ and $\bm{\varphi}^k$ from client $k$.  \label{23}
%                 \State Update table $\mathbf{E}$ by Eq. (\ref{eq:update E}). 
%                 \State Update vector $\bm{\Phi}$ by Eq. (\ref{eq:update phi}). \label{24}
% 	\end{algorithmic}
% \end{algorithm}

%\usepackage{algorithm}
% \begin{algorithm}[t]
% 	\caption{ Procedure of CoCa } \label{alg:CoCa}
% 	\begin{algorithmic}[1]
%         \State \textbf{Client side}:
%         \State Initialize DNN model with total $L$ cache layers, local timestamp vector $\bm{\tau}$ and local class frequency vector $\bm{\varphi}$.
%         \While {True}
%             \State Upload $\bm{\tau}$ and request cache.\label{4}
%             \State Initialize the cache update table $\mathbf{U}$.
%             \For{ $i=1$ to $F$ }
%                 \For{ $j=1$ to $L+1$ } 
%                     % \Statex \Comment{$L$ is the number of all cache layers}
%                     \State Process frame $i$ through model block $j$
%                     \If{cache layer $j$ available}
%                         \State Extract the semantic vector $\mathbf{V}_j$.
%                         \State Perform cache lookups.
%                         \If{ cache hits }
%                             \State Exit early.
%                         \EndIf
%                     \EndIf
%                 \EndFor
%                 \State Update $\bm{\tau}$, $\bm{\varphi}$.
%                 \State Update $\mathbf{U}$ by Eq. (\ref{eq:update U}).
%             \EndFor
%             \State Upload $\mathbf{U}$ and $\bm{\varphi}$ for the global updates. \label{16}
%         \EndWhile
%         % server
%         \State \textbf{Server side}: 
%         \State Initialize the DNN model, global class frequency vector $\bm{\Phi}$, and global cache table $\mathbf{E}$. 
%         \State Let $\mathcal{K} = \{1, 2, ..., N\}$ be the set of all clients
%         \While {True}
%             \For {each client  $k \in \mathcal{K}$ (in parallel)}
%                 \State Receive cache allocation request from client $k$, along with decision-support information, such as $\bm{\tau}^k$. \label{19}
%                 %\State  cache entry by Algorithm \ref{alg:cache select}.
%                 \State Allocate the proper cache to client $k$ by Alg. \ref{alg:cache select}.  \label{21}
%                 \State Wait for client $k$ to complete local inference
%                 \State Receive $\mathbf{U}^k$ and $\bm{\varphi}^k$ from client $k$.  \label{23}
%                 \State Update table $\mathbf{E}$ by Eq. (\ref{eq:update E}). 
%                 \State Update vector $\bm{\Phi}$ by Eq. (\ref{eq:update phi}). \label{24}
%             \EndFor
%         \EndWhile
% 	\end{algorithmic}
% \end{algorithm}

Now, we will describe the method for collecting semantic vectors.
For the selected inference sample of class $i$, its semantic vector at layer $j$ is denoted as $\mathbf{V}_{i,j}$, and the corresponding cache entry in the cache update table is denoted as $\mathbf{U}_{i,j}$. 
The entry $\mathbf{U}_{i,j}$ is first updated as follows:
\begin{equation}
    \mathbf{U}_{i,j} = \mathbf{V}_{i,j} + {\beta} \cdot \mathbf{U}_{i,j}
    \label{eq:update U}
\end{equation}
where ${\beta}$ is the decay coefficient (set to 0.95 by default), which attenuates the influence of older inference samples.
Then, $\mathbf{U}_{i,j}$ is normalized to have a unit L2 norm.
Upon completing local inferences and collecting update information, the client uploads the cache update table for global updates. The client continues to the next round, passing the task back to the server side.

% 一些缩写的全称要不不写了或者放在算法前面
% \begin{algorithm}[t]
% 	\caption{ Procedure of CoCa } \label{alg:CoCa}
% 	\begin{algorithmic}[1]
%         \State \textbf{Client side}:
%         \State Initialize DNN model (with total $L$ cache layers), local timestamp vector $\bm{\tau}$ and local class frequency vector $\bm{\varphi}$.
%         \While {True}
%             \State Upload $\bm{\tau}$ and request cache.\label{4}
%             \State Initialize the cache update table $\mathbf{U}$.
%             \For{ Each frame in $F$ frames }
%                 \For{ $j=1$ to $L+1$ } 
%                     % \Statex \Comment{$L$ is the number of all cache layers}
%                     \State forward with the model block $j$.
%                     \If{cache layer $j$ available}
%                         \State Extract the semantic vector $\mathbf{V}_j$.
%                         \State Cache lookups.
%                         \If{ Cache hits }
%                             \State Early exit.
%                         \EndIf
%                     \EndIf
%                 \EndFor
%                 \State Update $\bm{\tau}$, $\bm{\varphi}$.
%                 \State Update $\mathbf{U}$ by Eq. (\ref{eq:update U}).
%             \EndFor
%             \State Upload $\mathbf{U}$ and $\bm{\varphi}$ for the global updates. \label{16}
%         \EndWhile
%         \State \textbf{Server side}: 
%         \State Initialize the DNN model, global class frequency vector $\bm{\Phi}$, and global cache table $\mathbf{E}$.
%         \While {True}
%             \State Receive cache allocation request from client $k$, along with decision support information. \label{19}
%             \State Allocate cache by Algorithm \ref{alg:cache select}. \label{20}
%             \State Send the selected cache to client $k$. \label{21}
%             \State Perform local inferences.
%             \State Receive $\mathbf{U}^k$ and $\bm{\varphi}^k$ from client $k$. \label{23}
%             \State Update table $\mathbf{E}$ by Eq. (\ref{eq:update E}). 
%             \State Update vector $\bm{\Phi}$ by Eq. (\ref{eq:update phi}).\label{24}
%         \EndWhile
% 	\end{algorithmic}
% \end{algorithm}


% \vspace{-0.3cm}

\subsection{ Cache Allocation and Global Updates }

% The server in CoCa is primarily responsible for two functions: cache allocation (Lines \ref{19}-\ref{21}) and global updates (Lines \ref{23}-\ref{24} of Algorithm \ref{alg:CoCa}). 
The server in CoCa is primarily responsible for two functions: cache allocation and global updates. 
For cache allocation request of client $k$, the server allocates suitable cache entries from the global cache, based on the client status information collected (such as the local timestamp vector $\bm{\tau}^k$) and the global status information maintained on the server. Details of the cache allocation algorithm can be found in Section \ref{sec:algorithm}.
% 
% Taking the example depicted in Fig. \ref{fig:frame}, the server maintains a $5 \times 5$ two-dimensional global cache table. The five rows represent the five classification classes of the task, and the five columns correspond to the five pre-set cache exit layers in the model.
% Under a cache size threshold of ten entries (ignoring differences in the size of cache entries), client 1 is allocated the first and third cache columns, with four entries per layer (four hot-spot classes). Meanwhile, the client $N$ is allocated the first, third, and fourth cache layers, with three entries per layer (three hot-spot classes). During inference, the client model only performs cache lookup operations at the cache layers having the assigned cache entries.


Global updates primarily involve updating the global cache table and class frequency information. For global cache updates, both the global cache table and the cache update table uploaded from the clients have the same two-dimensional logical structure. 
% 
In CoCa, the global cache table is updated by element-wise weighted summation of the corresponding entries from the local cache update table and the global cache table, with weights based on local and global class frequencies.
For client $k$, we denote the entry in the local cache update table for class $i$ and cache layer $j$ as $\mathbf{U}^k_{i,j}$, and the entry in the global cache table as $\mathbf{E}_{i,j}$.
Corresponding to the local class frequency vector $\bm{\varphi}^k$, the global class frequency vector is denoted as $\bm{\Phi}$.
For the update information from client $k$, the global cache entry $\mathbf{E}_{i,j}$ is updated as follows:
\begin{equation}
    \mathbf{E}_{i,j} = {\gamma} \cdot \frac{ {\Phi}_{i} }{ {\Phi}_{i} + {\varphi}^k_{i} } \cdot \mathbf{E}_{i,j} + \frac{ {\varphi}^k_{i} }{ {\Phi}_{i} + {\varphi}^k_{i} } \cdot \mathbf{U}^k_{i,j}
    \label{eq:update E}
\end{equation}
where ${\Phi}_{i}$ and ${\varphi}^k_{i}$ represent the global total frequency and local frequency, respectively, for the samples of class $i$. 
The parameter ${\gamma}$ is the decay coefficient, and is set to 0.99 for subsequent experiments. Thus, we evaluate the importance of updating entries using their frequency and perform a weighted average. 
After updates, $\mathbf{E}_{i,j}$ is normalized to have a unit L2 norm.
% 
The global class frequency vector $\bm{\Phi}$ is updated by adding the local class frequency vector $\bm{\varphi}^k$ of client $k$. Mathematically, the update for each class $i$ is formulated as:
\begin{equation}
    {\Phi}_i = {\Phi}_i + {\varphi}^k_i
    \label{eq:update phi}
\end{equation}
The procedure outlined above describes how the server implements the updates of the global cache and state information.
%These update steps allow us to aggregate information from the clients into the global status information.
%The global class frequency vector simply requires a simple addition with the local class frequency vector to update itself. Through these update steps, we aggregate information from the client into the global status information.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/framework2.pdf}
  \caption{An illustrative example of CoCa. The server maintains a $5\times5$ global cache. For personalized cache allocation, client 1 is assigned cache entries in the 1st and 3rd layers, with four entries per layer, while client $N$ is assigned cache entries in the 1st, 3rd, and 4th layers, with three entries per layer.}
  \label{fig:frame}
\end{figure}

\textcolor{blue}{
\subsection{Illustrative Example of CoCa}
To illustrate our proposed framework CoCa, we take the example depicted in Fig. \ref{fig:frame}. 
The server maintains a $5 \times 5$ two-dimensional global cache table. The five rows represent the five classification classes of the task, and the five columns correspond to the five pre-set cache exit layers in the model.
Consider a scenario with a cache size threshold of ten entries, 
Client 1's recent data stream is heavily concentrated on four primary classes, which have more recent timestamps and higher frequencies compared to the infrequent appearance of other classes. 
Upon receiving Client 1's state information and cache request, the server allocates four entries per cache layer. 
Then, the server uses a greedy algorithm to sequentially select cache layers that maximize contribution. 
As a result, the server may provide Client $1$ with the first and third cache layers, each populated with four entries corresponding to the frequently accessed classes.
When the number of frequently accessed classes for Client $N$ decreases from four to three, the server adapts by selecting three cache layers (such as the first, third, and fourth layers), each containing three entries.
This approach dynamically accommodates the changing data patterns of clients. 
In CoCa, each client communicates solely with the server, eliminating the need for direct synchronization of cache updates and allocations between clients. 
Information sharing across clients is facilitated through the server’s global cache update mechanism.
}



% Under a cache size threshold of ten entries (ignoring differences in the size of cache entries), client 1 is allocated the first and third cache columns, with four entries per layer (four hot-spot classes). Meanwhile, the client $N$ is allocated the first, third, and fourth cache layers, with three entries per layer (three hot-spot classes). During inference, the client model only performs cache lookup operations at the cache layers having the assigned cache entries.

==> content/trash.tex <==
% In this section, we define the problem of heterogeneity-aware FL with adaptive neural compostion and gredient compression. Let $t_{i}^{k, cp}$ denote the computation time for local updating of client $i$ at round $k$, which is related to the size of coefficient obviously. The larger the coefficient is, the more parameters the composed model will have, leading to longer local computation time. Considering the upload speed is usually much smaller than the download speed in FL and the parameters download time is negligible, we focus on the gredients upload time. Suppose that the gredients size of shared basis and full coefficient are $B_{v}$ and $B_{u}$, respectively, the communication time of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cm} = \frac{r_{i}^{k} (B_{v} + p_{i}^{k} B_{u}) } {b_{i}^{k}}
% \end{equation}
% where $c_{i}^{k}$ represents the upload bandwidth of client $i$ at round $k$, which is heterogeneous among clients and can change dynamically in different rounds. We define the completion time of client $i$ at round $k$ as follows:
% \begin{equation}
%     t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}
% \end{equation}
% Due to the synchronization barrier of FL, the round time (\ie, duration between two successive
% training rounds) depends on the slowest client, which can be expressed as:
% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{N}} \ t_{i}^{k}
% \end{equation}

% Our goal is to determine the optimal coefficient pruning ratios and gredients compression ratios for each client every round, so as to accelerate the training process in the heterogeneous FL setting. Accordingly, we formulate the joint optimization problem as follows:

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \epsilon \\
%     p_{i}^{k} \in \mathcal{P}, &\forall i, \forall k \\
%     0 < r_{i}^{k} \leq  1, & \forall i, \forall k 
%     \end{cases}
% \end{equation}

% The first inequality expresses the convergence requirement, where $\epsilon$ (a positive constant close to zero) is the convergence threshold of the training loss after $K$ rounds. The second set of inequalities bounds the feasible range of coefficient pruning ratios, while the third set of inequalities bounds that of gredient compression ratios.

% In this section, we define the problem of heterogeneity-aware FL with adaptive client selection and neural composition. Let $g(x_{i}^{k, h}, p_{i}^{k})$ represent the number of CPU cycles required to perform one local update, which is related to the size of coefficient. The larger the coefficient is (\ie, the more parameters the composed model have), the more CPU cycles it required to process a batch of data samples. Thus, the computation the of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cp} = \frac{\sum_{h=1}^{H} g(x_{i}^{k, h}, p_{i}^{k})} {c_{i}^{k}}
% \end{equation}

% where $c_{i}^{k}$ denote the CPU-cycle frequency for local training in round $k$. For the communication time, considering the upload speed is usually much smaller than the download speed in FL and the parameters download time can be negligible, we focus on the upload time. Suppose that the size of shared basis and full coefficient are $B_{v}$ and $B_{u}$, respectively, the communication time of client $i$ at round $k$ can be formulated as follows:

% \begin{equation}
%     t_{i}^{k, cm} = \frac{(B_{v} + p_{i}^{k}B_{u}) } {b_{i}^{k}}
% \end{equation}

% where $c_{i}^{k}$ represents the upload bandwidth of client $i$ at round $k$, which is heterogeneous among clients and can change dynamically in different rounds. Due to the synchronization barrier of FL, the round time (\ie, duration between two successive training rounds) depends on the slowest client, which can be expressed as:

% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{M}^{k}} \ t_{i}^{k}
% \end{equation}


% where $t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}$. Our goal is to select the clients involved in FL based on the statistical heterogeneity and determine the optimal size of coefficient for those selected clients, so as to accelerate the training process in the heterogeneous FL setting. Accordingly, we formulate the joint optimization problem as follows:

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \epsilon \\
%     p_{i}^{k} \in \mathcal{P}, &\forall i, \forall k \\
%     |\mathcal{M}^{k}| = M, & \forall k 
%     \end{cases}
% \end{equation}

% The first inequality expresses the convergence requirement, where $\epsilon$ (a positive constant close to zero) is the convergence threshold of the training loss after $K$ rounds. The second set of inequalities bounds the feasible range of coefficient pruning ratios. The third set of inequalities indicates that the PS selects $M$ clients participating in training at each round.

% $c_{i}^{p}$ is the computing resource consumption of one local iteration.
% $b_{v}$ and $b_{u}$

% \begin{equation}
%     t_{i}^{k, cp} = \frac{\sum_{h=1}^{\tau_{i}^{k}} g(x_{i}^{k, h}, p_{i}^{k})} {c_{i}^{k}}
% \end{equation}

% \begin{equation}
%     t_{i}^{k, cm} = \frac{(B_{v} + p_{i}^{k}B_{u}) } {b_{i}^{k}}
% \end{equation}

% \begin{equation}
%     t^{k} = \mathop{\max}_{i \in \mathcal{N}} \ t_{i}^{k}
% \end{equation}

% \begin{equation}
%     t_{i}^{k} = t_{i}^{k, cp} + t_{i}^{k, cm}
% \end{equation}

% \begin{equation}
%     \mathcal{W}^{k} = \frac{1}{N} \sum_{i = 1}^{N} (t^{k} - t^{k}_{i})
% \end{equation}

% \centerline{$\mathop{\min} \sum_{k=1}^{K} t^{k}$}
% \begin{equation}
%     s.t.
%     \begin{cases}
%     F(\omega^{K}) - F(\omega^{*}) \leq \xi  \\
%     \sum_{k = 1}^{K} \sum_{i = 1}^{N} (b_{i, v} + b_{i, u} \cdot p_{i}^{k}) \leq B  \\
%     \sum_{k = 1}^{K} \sum_{i = 1}^{N} \tau_{i}^{k} \cdot p_{i}^{k}c_{i} \leq C 
%     \end{cases}
% \end{equation}


% t_{i}^{k} = \frac{\tau_{i}^{k} g(V^{k} \cdot U^{k}_{p_{i}})} {c_{i}^{k}} + \frac{h(V) + h(U^{k}_{p_{i}}) } {b_{i}^{k}}, & \forall i, k \\

% \subsection{Federated Learning Basics}
% Consider a loose federation of $N$ clients $\mathcal{N} = \{1, 2, \cdots, N \}$ coordinated by the PS.
% Each client $n \in \mathcal{N}$ holds its local dataset $D_{n} = \{\zeta_{i}^{n}\}_{i=1}^{|D_{n}|}$, where $\zeta_{i}$ denotes a data sample from $D_{n}$.
% Further, we represent the loss function as $\mathcal{L}(\mathbf{x}; \zeta)$, which measures how well the model $\mathbf{x}$ perform on data sample $\zeta$.
% Therefore, the local loss function of client $n$ is defined as:

% \begin{equation}
%     F_{n}(\mathbf{x}) \triangleq \mathbb{E}_{\zeta \thicksim D_{n}} [\mathcal{L}(\mathbf{x}; \zeta)] 
% \end{equation}

% The global loss function is a linear combination of all $N$ clients, and the goal of FL is to train a high-quality model $\mathbf{x}^{*}$ to minimize the value of global loss function, which can be defined as follows:

% \begin{equation} \label{eq:fl_goal}
%     \mathbf{x}^{*} \triangleq  \mathop{\arg\min}_{\mathbf{x}} F(\mathbf{x}) = \mathop{\arg\min}_{\mathbf{x}} \frac{1}{N} \sum_{n=1}^{N} F_{n} (\mathbf{x})
% \end{equation}

% FedAvg \cite{mcmahan2017communication} is the pioneer and also the most widely used FL method to solve the problem in Eq. \eqref{eq:fl_goal}.
% In each round $h \in \{1, 2, \cdots, H\}$, the PS randomly selects $K$ clients to participate in training and sends the global model $\mathbf{x}^{h}$ to the selected clients $\mathcal{N}^{h} \subseteq  \mathcal{N}$.
% Then, each client $n \in \mathcal{N}^{h}$ performs local update for $\tau$ iterations.
% Let $\mathbf{x}^{h}_{n} (t)$ denote the local model of client $n$ at iteration $t$ in round $h$.
% For the mini-batch stochastic gradient descent (SGD) algorithm, a local update step can be expressed as follows:

% \begin{equation}
%     \mathbf{x}^{h}_{n} (t+1) = \mathbf{x}^{h}_{n} (t) - \eta \nabla F_{n} (\mathbf{x}^{h}_{n} (t); \xi_{n}^{h, t})
% \end{equation}
% where $\xi_{n}^{h, t}$ denotes a random data batch from the local dataset $D_{n}$ and $\eta$ is the learning rate.
% Finally, the PS collects the updated model $\mathbf{x}^{h}_{n}$ from the participating clients and aggregate them to the latest global model for further training, \ie, $ \mathbf{x}^{h+1} = \frac{1}{N} \sum_{n=1}^{N} \mathbf{x}^{h}_{n} (\tau) $.




% \subsection{Impact of model width}

% As the most common terminal device, mobile phones are the primary data source and usually participate in training as clients.
% However, in practice, these phones are generally resource-constrained with poor computing power, so that they may not be able to afford the overhead to train the complete model.
% Therefore, it is necessary to reduce the model complexity for these poor clients, which can be achieved by reducing the model's depth (\ie, number of layers) or width (\ie, number of hidden channels) \cite{diao2020heterofl, horvath2021fjord, kim2023depthfl}.
% In this work, we adjust the model complexity by modulating the model width, which can reduce parameters and memory footprint during training more effectively compared to reduing model depth \cite{mei2022resource}.

% We can significantly reducing the computing complexities and training overhead of a DNN model, but it usually comes with performance degradation.
% To verify this phenomenon, we construct a CNN model with three 3$\times$3 convolutional layers and one fully-connected layer.
% We reduce the number of hidden channels in each layer by 0.25, 0.5, 0.75 and 1.0 times, respectively, and train these models in different width over CIFAR-10 to record their training overhead and test accuracy.
% The results shown in Table. xx indicate that the smaller the model width, the less training overhead, but the lower the accuracy.
% For instance, xxxx.
% To minimize the performance degradation, the model width should be as large as possible within the clients' computing power.

% \begin{table}[h]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_with}
% 	\begin{tabular}{c|ccc}
% 		\hline
% 		Width & \tabincell{c}{Memory \\ Footprint (MB)} & FLOPs (M) & \tabincell{c}{Test \\ Accuracy (\%)} \\
% 		\hline
% 		0.25$\times$ & -- & -- & -- \\
% 		0.5$\times$  & -- & -- & -- \\
% 		0.75$\times$ & -- & -- & -- \\
% 		1.0$\times$  & -- & -- & -- \\
% 		\hline
% 	\end{tabular}
% \end{table}
% % To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} propose to prune the global model into a small one.
% % Nevertheless, the pruned parameters cannot be optimized on client's local data, resulting in poor performance.

% % In order to reduce the model complexity without much performance degradation, we decompose the model into two low-rank tensors, named neural basis and coefficient, and only prune the coefficient.
% % The entire neural basis is trained by all clients and the update can be propagated to every model parameter after recomposition, ensuring high model performance.
% % To varify the effectiveness of the proposed approach, we train the models in different complexities (\ie, GPU memory occupancy) over ImageNet-100.
% % The results shown in Fig. \ref{fig:motivation_acc_memory} indicate that the smaller the model, the worse the performance (\ie, accuracy).
% % Besides, it can be observed that the composited model achieves about 5.1\% higher accuracy than the pruned model at the same computing complexity. 

% % There is still one issue when .
% % According to related research, most people use cheap mobile phones with low computing power.
% % Therefore, most clients can only train a small part of coefficient, resulting that the total updating time varies greatly between different coefficient parts.
% % This training inconsistency in updating times may have a negative impact on the convergence performance.
% % We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% % The results in Fig. \ref{fig:motivation_acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% % To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:motivation_acc_hetero}.





% % In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}. 
% % However, the computing capabilities of each clinet may vary significantly and even dynamically in practice \cite{diao2020heterofl}.

% % In practice, the computing capabilities of clients may significantly heterogeneous and even vary dynamically \cite{diao2020heterofl}.

% % In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}, which means a same computational complexity for all clients.
% % Nevertheless, the computing capabilities of clients are generally heterogeneous and may even change dynamically in practice, leading to a long system waiting time in synchronous manner \cite{xu2022adaptive}.
% % Moreover, as the model size continues to increase (\eg, the parameters number of GPT-3 reaches 175 billion \cite{floridi2020gpt}), resource-constrained edge clients may not be able to afford the training overhead (\eg, memory, energy).
% % To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} prune or quantify the global model into a submodel for each client based on its computing capability, so as to alleviate the synchronization barrier issue and diminish the resource consumption.
% % However, for the prune-based methods, the unpruned parameters cannot be optimized in clients' local data, leading to poor performance of global model.
% % Besides, the quantify-based methods will introduce model errors, which also diminishes the performance.
% % Instead of pruning the global model into local ones, FLANC \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% % construct models at various complexities by composing different neural components (\ie, tensors).
% % Instead of pruning or 

% % Different from the above methods, Flanc \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% % The neural basis is trained by all participating clients and the updating can be propagated to every model parameter through neural composition.
% % We trained models in different complexities (\ie, GPU memroy usage) over ImageNet-100 by HeteroFL and Flanc, respectively. 
% % The results shown in Fig. \ref{fig:acc_memory} indicate that the composited model can achieve higher accuracy compared to the pruned model with the same complexity.

% % \begin{figure}[h]
% % 	\centering
% % 	\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}
% % 	\caption{Model performance of different methods.}\label{fig:acc_memory}
% % 	\vspace{-3mm}
% % \end{figure}

% % \begin{figure}[h]
% % 	\centering
% % 	\subfigure[Different computing complexities]{
% % 		\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}\label{fig:motivation_acc_memory}
% % 	}
% % 	\subfigure[Different hetergeneity levels]{
% % 		\includegraphics[width=1.6in]{fig/motivation_acc_hetero.pdf}\label{fig:motivation_acc_hetero}
% % 	}
% % 	\caption{The model accuracy in different conditions.}\label{fig:motivation_model_accuracy}
% % 	\vspace{-3mm}
% % \end{figure}






% \subsection{Impact of local update frequency}
% % Even if FLANC \cite{mei2022resource} enables clients to train complexity-adjustable model.
% % In general, the above techniques are able to custom the model's computing complexity according to clients' computing power.
% % There is still one issue to perform FL in edge computing system.
% % By pruning the coefficient, we can custom the model's computing complexity according to clients' computing power.
% % However, there is still one issue to 
% % However, the edge clients are not only heterogeneous in terms of computing capability, but also in terms of communication capability (\eg, bandwidth) \cite{wang2022accelerating}.
% % As shown in Fig. \ref{fig:round_time_noadloc}, although the local updating time is approximately equal among all clients, the clients with slow communication speed can easily become the bottleneck and lead to long idle time for fast clients. 

% There is still one issue to perform FL in edge computing system.
% Since the clients' capabilities (\eg, computing power, bandwidth) are highly heterogeneous and even time-varying, the stragglers will delay the aggregation and result in long idle time for fast clients.
% As shown in Fig. \ref{fig:round_time_noadloc}, the time cost of the fastest client in one round is only 20\% of the slowest client.
% In other word, 80\% of the fastest client' time is wasted.

% In order to alleviate this problem, we can adjust the numbers of local iterations for different clients, and the effect is illustrated in Fig. \ref{fig:round_time_adloc}.
% On the one hand, the slower can perform fewer local iterations to reduce the impact of stragglers.
% On the other hand, the faster clients can utilize the idle time to perform more local iterations, which helps the model converge faster.
% However, the models trained with different number of local iterations are discrepant, which may affect the convergence performance of global model, especially when the local models' architecture are different.
% Therefore, the existing algorithms to adjust the number of local iterations \cite{wang2018edge} cannot be directly applied in our work. 

% \begin{figure}[h]
% 	\centering
% 	\subfigure[Fixed Updating Frequency]{
% 		\includegraphics[width=1.6in]{fig/motivation_roundtime_noadloc.pdf}\label{fig:round_time_noadloc}
% 	}
% 	\subfigure[Adaptive Updating Frequency]{
% 		\includegraphics[width=1.6in]{fig/motivation_round_adloc.pdf}\label{fig:round_time_adloc}
% 	}
% 	\caption{Ranked clients' time cost in one round.}\label{fig:round_time}
% 	\vspace{-3mm}
% \end{figure}

% % There is still one issue when trianing complexity-adjustable in mobile phones.
% % According to related research, most people use cheap mobile phones with low computing power.
% % Therefore, most client can only train a small part of coefficient, which results that the updating time varies greatly between different clients.
% % This training inconsistency may have a negative impact on the convergence performance.
% % We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% % The results in Fig. \ref{fig:acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% % To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:acc_hetero}.

% However, running these models on edge clients (\eg, smartphones) may encounter performance degradation issues due to the limited computational and communication resources. 

% As the most common terminal device, mobile phones are the primary data source and usually participate in training as clients.
% However, in practice, these phones are generally resource-constrained with poor computing power, so that they may not be able to afford the overhead to train the complete model.

% \begin{table}[t]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_with}
% 	\begin{tabular}{c|ccccc}
% 		\hline
% 		Width & Parameters(M) & Size(MB) & \tabincell{c}{Memory \\ Footprint(MB)} & FLOPs(M) & \tabincell{c}{Test \\ Accuracy(\%)} \\
% 		\hline
% 		0.25$\times$ & -- & -- & -- & -- & -- \\
% 		0.5$\times$  & -- & -- & -- & -- & -- \\
% 		0.75$\times$ & -- & -- & -- & -- & -- \\
% 		1.0$\times$  & -- & -- & -- & -- & -- \\
% 		\hline
% 	\end{tabular}
% \end{table}

% To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} propose to prune the global model into a small one.
% Nevertheless, the pruned parameters cannot be optimized on client's local data, resulting in poor performance.

% In order to reduce the model complexity without much performance degradation, we decompose the model into two low-rank tensors, named neural basis and coefficient, and only prune the coefficient.
% The entire neural basis is trained by all clients and the update can be propagated to every model parameter after recomposition, ensuring high model performance.
% To varify the effectiveness of the proposed approach, we train the models in different complexities (\ie, GPU memory occupancy) over ImageNet-100.
% The results shown in Fig. \ref{fig:motivation_acc_memory} indicate that the smaller the model, the worse the performance (\ie, accuracy).
% Besides, it can be observed that the composited model achieves about 5.1\% higher accuracy than the pruned model at the same computing complexity. 

% There is still one issue when .
% According to related research, most people use cheap mobile phones with low computing power.
% Therefore, most clients can only train a small part of coefficient, resulting that the total updating time varies greatly between different coefficient parts.
% This training inconsistency in updating times may have a negative impact on the convergence performance.
% We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% The results in Fig. \ref{fig:motivation_acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:motivation_acc_hetero}.


% In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}. 
% However, the computing capabilities of each clinet may vary significantly and even dynamically in practice \cite{diao2020heterofl}.

% In practice, the computing capabilities of clients may significantly heterogeneous and even vary dynamically \cite{diao2020heterofl}.

% In FL, each client's local model shares the same architecture \cite{mcmahan2017communication}, which means a same computational complexity for all clients.
% Nevertheless, the computing capabilities of clients are generally heterogeneous and may even change dynamically in practice, leading to a long system waiting time in synchronous manner \cite{xu2022adaptive}.
% Moreover, as the model size continues to increase (\eg, the parameters number of GPT-3 reaches 175 billion \cite{floridi2020gpt}), resource-constrained edge clients may not be able to afford the training overhead (\eg, memory, energy).
% To this end, most existing works \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex, kim2023depthfl} prune or quantify the global model into a submodel for each client based on its computing capability, so as to alleviate the synchronization barrier issue and diminish the resource consumption.
% However, for the prune-based methods, the unpruned parameters cannot be optimized in clients' local data, leading to poor performance of global model.
% Besides, the quantify-based methods will introduce model errors, which also diminishes the performance.
% Instead of pruning the global model into local ones, FLANC \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% construct models at various complexities by composing different neural components (\ie, tensors).
% Instead of pruning or 

% Different from the above methods, Flanc \cite{mei2022resource} employs low-rank approximation to represent models in different complexities.
% The neural basis is trained by all participating clients and the updating can be propagated to every model parameter through neural composition.
% We trained models in different complexities (\ie, GPU memroy usage) over ImageNet-100 by HeteroFL and Flanc, respectively. 
% The results shown in Fig. \ref{fig:acc_memory} indicate that the composited model can achieve higher accuracy compared to the pruned model with the same complexity.

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}
% 	\caption{Model performance of different methods.}\label{fig:acc_memory}
% 	\vspace{-3mm}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	\subfigure[Different computing complexities]{
% 		\includegraphics[width=1.6in]{fig/motivation_acc_memory.pdf}\label{fig:motivation_acc_memory}
% 	}
% 	\subfigure[Different hetergeneity levels]{
% 		\includegraphics[width=1.6in]{fig/motivation_acc_hetero.pdf}\label{fig:motivation_acc_hetero}
% 	}
% 	\caption{The model accuracy in different conditions.}\label{fig:motivation_model_accuracy}
% 	\vspace{-3mm}
% \end{figure}

% Even if FLANC \cite{mei2022resource} enables clients to train complexity-adjustable model.
% In general, the above techniques are able to custom the model's computing complexity according to clients' computing power.
% There is still one issue to perform FL in edge computing system.
% By pruning the coefficient, we can custom the model's computing complexity according to clients' computing power.
% However, there is still one issue to 
% However, the edge clients are not only heterogeneous in terms of computing capability, but also in terms of communication capability (\eg, bandwidth) \cite{wang2022accelerating}.
% As shown in Fig. \ref{fig:round_time_noadloc}, although the local updating time is approximately equal among all clients, the clients with slow communication speed can easily become the bottleneck and lead to long idle time for fast clients. 
% There is still one issue to perform FL in edge computing system.
% Since the clients' capabilities (\eg, computing power, bandwidth) are highly heterogeneous and even time-varying, 

% As shown in Fig. \ref{fig:round_time_noadloc}, the time cost of the fastest client in one round is only 20\% of the slowest client.

% There is still one issue when trianing complexity-adjustable in mobile phones.
% According to related research, most people use cheap mobile phones with low computing power.
% Therefore, most client can only train a small part of coefficient, which results that the updating time varies greatly between different clients.
% This training inconsistency may have a negative impact on the convergence performance.
% We run Flanc over ImageNet-100 on different heterogeneity level, which is the proportion of clients with low computing power among all clients.
% The results in Fig. \ref{fig:acc_hetero} shows that, the higher the heterogeneity level, the more training inconsistent and the lower the accuracy.
% To this end, we can also adjust the local updating frequencies for different coefficient parts to ensure the consistency, which is confirmed by the result in Fig. \ref{fig:acc_hetero}.

% Moreover, the heterogeneity among the clients, \ie, the computing power and communication capacity of different edge clients is significantly varied, will also have a great impact on training efficiency.
% For example, the hardware manufacturer typically configure 
% For example, mobile manufacturers typically configure multiple processors (\eg, Snapdragon, Apple A-series chips) on the client to cater to the diverse needs of customers, however, resulting in inconsistent completion time for model training.
% Besides, the computing power and communication capacity of different edge clients is significantly varied, which will have a great impact on training efficiency.
% For example, there can be a tenfold difference in CPU frequency or bandwidth for the edge devices \cite{xu2022adaptive}.
% In synchronous mode, clients with faster training and/or communication speed often have to wait the stragglers for global aggregation, resulting in a longer or even unacceptable completion time of model training.
% In addition, due to the intrinsic and/or external conditions, such as ambient temperatures, CPU states,
% network connections to the server and so on, the per-round computing time and communication time at each client may vary significantly.
% The different network connection methods (\eg, 4G, 5G and WIFI) of the client also affect the communication cost of model transmission during the training process\cite{}.
% Besides, the availability and connectivity of edge clients may change over time, \ie, network dynamics.
% For instance, the smartphone can freely join or exit the training process. 
% The addition of clients will increase the scale and data diversity of training, while the withdrawal of clients may lead to data loss during training, leading to the performance degradation of the model training.

% Moreover, the heterogeneity among the clients, \ie, the computing power and communication capacity of different edge clients is significantly varied, will also have a great impact on training efficiency.
% For example, the hardware manufacturer typically configure 
% For example, mobile manufacturers typically configure multiple processors (\eg, Snapdragon, Apple A-series chips) on the client to cater to the diverse needs of customers, however, resulting in inconsistent completion time for model training.

% The different network connection methods (\eg, 4G, 5G and WIFI) of the client also affect the communication cost of model transmission during the training process\cite{}.
% Besides, the availability and connectivity of edge clients may change over time, \ie, network dynamics.
% For instance, the smartphone can freely join or exit the training process. 
% The addition of clients will increase the scale and data diversity of training, while the withdrawal of clients may lead to data loss during training, leading to the performance degradation of the model training.

% For example, performing one mini-batch SGD on standard ResNet-18\footnote{Image resolution is 3$\times$144$\times$144, batch size is 32.} with NVIDIA Jetson TX2\footnote{A commercial edge embedded AI computing device. More details are available at https://www.nvidia.cn/autonomous-machines/embedded-systems} takes xxx minutes and consumes xx\% of the battery.


% Different from pruning the global model directly, \textit{Flanc} \cite{mei2022resource} proposes to construct the models in different width by multiplying the neural basis with different coefficient.
% The neural basis is shared by all clients, which enables every parameter in global model to access the full range of knowledge of all clients, improving the performance of global model.
% Despite the improvement, \textit{Flanc} only aggregates the coefficients with the same shape, thus the learned coefficient will be biased towards the data distribution of corresponding particular clients set, which hurts the generalization performance of the global model when the local datasets are Non-IID.
% To verify this phenomenon, we test the \textit{HeteroFL} and \textit{Flanc} by training CNN on CIFAR-10 under three different Non-IID levels, denoted by \textit{low}, \textit{medium} and \textit{high}, respectively. 
% The results shown in Table \ref{table:motivation_training_heterogeneous_models} indicate that \textit{Flanc} achieves better performance than \textit{HeteroFL}, but the test accuracies of both \textit{Flanc} and \textit{HeteroFL} are significantly decreased as the Non-IID level increases.
% To this end, we design a novel neural composition technique to aggregate the coefficients in different shape into a global one and let the parameter in global coefficient be evenly trained, so as to improve the training robustness against Non-IID data.
% By Table \ref{table:motivation_training_heterogeneous_models}, the global model can achieve the best test accuracy with our proposed technique. 


% Therefore, it is necessary to reduce the model complexity for these resource-constrained clients by reducing the model's depth (\ie, number of layers) \cite{kim2023depthfl} or width (\ie, number of hidden channels) \cite{diao2020heterofl, horvath2021fjord, alam2022fedrolex}.
% In this work, we mainly focus on adjusting the model complexity by modulating the model width, which can reduce parameters and memory footprint during raining more effectively compared to reducing model depth \cite{mei2022resource}.

% Some techniques (\eg, model pruning) can significantly reduce the computing complexities and training overhead of a DNN model, but it usually comes with performance degradation.
% Reducing the model width can significantly reduce the computing complexities and training overhead, but it usually comes with performance degradation.
% To evaluate the impact of model width on FL training, we construct a CNN model with three 3$\times$3 convolutional layers and one fully-connected layer, where each convolutional layer has 64, 128 and 128 hidden channels, respectively.
% We reduce the model width by 0.25, 0.5, 0.75 and 1.0 times, and record the model's training overhead and test accuracy over CIFAR-10, respectively.
% The results in Table. \ref{table:motivation_models_in_different_width} indicate that the smaller the model width, the less training overhead, but the lower the accuracy.
% For instance, the 1.0-width model needs about 15 times more FLOPs to process an image than the 0.25-width model, but its test accuracy is 6.29\% higher.
% To minimize the performance degradation, the model width should be as large as possible within the clients' computing power.

% \begin{table}[t]
% 	\centering
% 	\setlength{\abovecaptionskip}{10pt}%
%     \setlength{\belowcaptionskip}{0pt}%
%     \footnotesize
% 	\caption{Comparison of models in different width.}
%     \label{table:motivation_models_in_different_width}
% 	\begin{tabular}{c|cccc}
% 		\hline
% 		Width & 0.25$\times$ & 0.5$\times$ & 0.75$\times$ & 1.0$\times$ \\
% 		\hline
% 		Parameters(K) & 34.87 & 97.29 & 187.4 & 305.16 \\
% 		Size(MB) & 0.13 & 0.37 & 0.72 & 1.16 \\
% 		Memory Footprint(MB) & 22.35 & 59.64 & 68.69 & 92.16 \\
% 		FLOPs(M) & 7.68 & 29.52 & 65.51 & 115.65 \\
% 		Test Accuracy(\%) &  81.09 & 85.05 & 86.65 & 87.38 \\
% 		\hline
% 	\end{tabular}
% \end{table}


==> his/Back_Related3.tex <==
\subsubsection{Edge Inference}
Traditional machine learning (ML) inference has primarily been offloaded to centralized cloud servers, taking advantage of their substantial processing resources \cite{alfakih2020task, chen2022context, zhang2021elf}. However, contemporary concerns regarding data privacy and the increasing demand for minimal inference latency have catalyzed a new trend. 
Edge devices (or clients), such as mobile phones, are emerging as feasible platforms for executing inference tasks, thus eliminating the need to offload these computations to the cloud. This migration shifts the focus of the inference from the cloud to the edge.
In the realm of edge inference, mobile vision processing tasks such as virtual/augmented reality and autonomous driving, with image classification as a predominant domain, have garnered significant focus.
Deep neural networks (DNNs) lead the forefront of models for various computer vision tasks, exhibiting widespread utility in diverse edge inference scenarios. 
With the advancement of the IoT and edge intelligence, research focus has gradually shifted from merely accelerating inference processes to optimizing inference under multi-client settings.


Existing research has increasingly concentrated on optimizing model executions to enhance inference speed in edge devices, exploring a variety of optimization strategies \cite{guo2018foggycache, cheng2017quantized, chen2021accelerating}. 
A prevalent strategy involves reducing the computational workload per inference through model compression, which accelerates the inference process. 
For instance, Cheng \etal \cite{cheng2017quantized} demonstrate that weight quantization can significantly mitigate the storage and computational burdens of models, thus reducing inference latency. However, this type of model compression might compromise the model's ability to classify accurately, particularly in complex tasks, potentially leading to notable losses in accuracy.
To address these issues, researchers have proposed methods such as model partitioning and edge-cloud collaborative inference. These approaches aim to prevent a decrease in inference accuracy and reduce transmission latency compared to pure cloud offloading methods.
Chen \etal \cite{chen2021accelerating} propose a scheme to dynamically partition DNN into two or three parts and distribute them at the edge and cloud, achieving the lowest delay with the change of request rate. 
These methods typically focus on point-to-point collaboration between individual clients and cloud servers, overlooking collaboration and comprehensive optimization of multiple clients. Moreover, employing segmented inference methods introduces privacy risks, as intermediate results may still be vulnerable to privacy leakage during transmission between the edge and the cloud.
To address these challenges, some multi-client collaborative systems have been proposed.
For example, FoggyCache \cite{guo2018foggycache} proposes cross-device approximate computation reuse, which minimizes redundant computation by harnessing the "equivalence" between different inputs and reusing previously computed outputs with high confidence.
The server acts as a coordinator, responsible for collecting reusable samples from various clients and providing support for reuse lookups.



\subsubsection{Caching in DNN}

Using cache in DNN model inference is a common method to reduce inference latency and improve long-term throughput. This approach stems from a crucial observation regarding the temporal locality often present in continuous vision tasks \cite{huynh2017deepmon, xu2018deepcache}. Such tasks frequently exhibit a pronounced temporal coherence among consecutive images within a video stream, where successive frames often manifest high similarity and correlation in their content and resultant classifications. For instance, in a video sequence, a particular object type may persist across numerous frames before vanishing, attributable to factors such as the mobile device (\eg, a smartphone) being in slow motion or stationary. To capitalize on this temporal locality inherent in continuous vision tasks, a straightforward approach involves the incorporation of caching. 
% 如何运用cache
Caching in DNN models typically involves inserting caches at the entry or intermediate layers of the model. When inference reaches the cache, it looks for one or more of the most similar entries. If the cache hit occurs, the inference result is determined based on their results through voting.


Extensive scholarly research on caching mechanisms for DNN models has produced varied proposals.
on one hand, work such as DeepCache \cite{xu2018deepcache} aim to reduce the computational load of current inference processes by reusing previously computed results. The pioneering work of DeepMon \cite{huynh2017deepmon} introduces the concept of using caching to accelerate inference tasks in video streams.
These methods leverage the characteristics of convolutional layers to cache the inference data from previous frames, block matching, and reuse intermediate results from similar regions. However, they face challenges such as high model coupling and complexity of implementation.
% 
On the other hand, some work \cite{fang2019teamnet, fang2020cachenet, ogden2021many} treat the model as a caching object to reduce the coupling between optimization methods and the model. For example, CacheNet \cite{fang2020cachenet} utilizes lightweight submodels as cache objects, dynamically replacing the model for inference based on input data. However, they may incur significant communication overhead during cache replacement.
% 
To address these issues, approximate-key caching and similar approaches \cite{finamore2022accelerating, li2021boosting} attempt to reduce the memory footprint of cache entries. For example, inspired by human cognitive patterns, SMTM \cite{li2021boosting} proposes an innovative semantic caching mechanism that uses low-dimensional representations of intermediate inference results as matching objects, thereby reducing the size of cache entries. 
% 
Nevertheless, there are still many aspects to be optimized when these methods encounter some challenges, such as non-IID data or long-tail distribution.



==> his/abstract3.tex <==
Edge inference is a technology that enables real-time data processing and analysis on clients near the data source. 
To ensure Quality of Service (QoS), such as low response latency, caching is used to reduce redundant computations in visual inference tasks. 
Sharing cache information among nearby clients can enhance performance due to task and data correlations. 
However, in a multi-client scenario, non-independent and identically distributed (non-IID) and long-tail distributions can reduce cache hit ratios and increase latency.
To address these challenges, we propose COLA, which adopts an efficient multi-client collaborative caching mechanism for enhancing edge inference performance. 
On the client side, the model is pre-set with multiple inactive cache layers for early exits. During inference, the model performs sequential lookups at cache layers activated by the server. 
On the server side, COLA uses a two-dimensional global cache to periodically aggregate information from each client, mitigating non-IID data effects.
% 微妙
For client cache allocation, COLA first evaluates class importance based on the frequency and recency of their samples. It then selects hot-spot classes to address long-tail distribution challenges. Finally, COLA dynamically activates cache layers to balance lookup overhead and accuracy.
Extensive experiments demonstrate that COLA can reduce inference latency by 23.0\%-45.2\% on the VGG and ResNet models with acceptable accuracy loss.

% Extensive experiments on real-world scenarios demonstrate that COLA reduces inference latency by 23.0\%-45.2\% on VGG and ResNet models, achieving a 1.1-1.3× increase in inference throughput compared to SOTA baselines with acceptable accuracy loss.

==> his/algorithm3.tex <==
\subsection{Problem Formulation}

% 
In this section, we define the cache entries selection optimization problem in our proposed framework, CoCa. The goal is to minimize average inference latency under constraints of cache size and inference accuracy loss on the client side through optimal allocation of cache entries.
% 
Assuming there are $\mathbf{N}$ clients, we need to allocate cache entries for each client from the global cache table. The global cache table consists of $\mathbf{I}$ rows and $\mathbf{L}$ columns, where $\mathbf{I}$ represents the total number of distinct classes in classification tasks, and $\mathbf{L}$ represents the maximum number of cache layers.
% 
Let $\mathbf{x}_{i,j}^k$ denote the allocation status of the cache entry in row $i$ and column $j$ for client $k$, where $\mathbf{x}_{i,j}^k \in {0, 1}$ for $0 < i \leq \mathbf{I}$, $0 < j \leq \mathbf{L}$, and $0 < k \leq \mathbf{N}$.
The size of the local cache is directly affected by the allocation status $\mathbf{x}_{i,j}^k$. Specifically, $\mathbf{x}_{i,j}^k = 1$ indicates that the corresponding cache entry is allocated, while $\mathbf{x}_{i,j}^k = 0$ means it is not. Therefore, the total size of the local cache is calculated by summing the sizes of all allocated cache entries.
Considering the varying sizes of the entries in different cache layers, we formulate the local cache size for client $k$ as follows:
\begin{equation}
    \mathbf{M}^k = \sum_{0 < i \leq \mathbf{I}, 0 < j \leq \mathbf{L}} \mathbf{x}_{i,j}^k \cdot \mathbf{m}_{i,j}
\end{equation}
where $\mathbf{m}_{i,j}$ represents the size of the entry in row $i$ and column $j$ of the cache table, \ie, the cache entry of class $i$ at layer $j$.


During inference, when the cache hits, the inference result corresponds to the class of the cache entry hit. Consequently, increasing the number of stored entries in the cache enhances the likelihood of the correct class being present. This, in turn, reduces the inference errors arising from cache hits where the correct class entries are absent, thereby decreasing the loss in inference accuracy.
on one hand, the accuracy loss is influenced by the number of entries per cache layer, which is related to the value of $\mathbf{X}^k$. The inference accuracy loss of client $k$ is denoted by $\mathcal{G}^k(\mathbf{X}^{k}, \bm{\Theta}^k)$, where $\mathbf{X}^{k}$ represents the set of all $\mathbf{x}_{i,j}^k$ values for client $k$, and $\bm{\Theta}^k$ denotes the cache hit thresholds for client $k$. 
Given the complexity of deriving an exact formula for $\mathcal{G}^k(\mathbf{X}^{k}, \bm{\Theta}^k)$, we estimate and characterize this relationship using empirical data obtained from server-side testing on a shared dataset.
% 这句话可能需要更详细的解释（需要解释这个函数的具体变化形式么）
% 
On the other hand, $\mathbf{x}_{i,j}^k$ is positively correlated with cache size, leading to increased inference time $\mathcal{C}_{j}(\mathbf{x}^{k})$ at layer $j$ of the model. 
This is straightforward to understand: more allocated cache entries (\ie, more $\mathbf{x}_{i,j}^k$ set to 1), both the number of cache layers and the number of entries per layer that need to be looked up also increase. Consequently, this leads to higher computational costs for cache lookup.
$\mathbf{L}$ cache layers divide the model into $\mathbf{L+1}$ model blocks. Therefore, we formulate the inference time for client $k$ as:
\begin{equation}
    \mathcal{T}^k(\mathbf{W}^k) = \sum_{j=1}^{\mathbf{L+1}} (1-\mathcal{P}_{j}(\mathbf{X}^{k}, \bm{\Theta}^k)) \cdot (\bm{\Lambda}_{j} + \mathcal{C}_{j}(\mathbf{X}^{k}))
\end{equation}
 

When allocating the local caches, CoCa selects appropriate cache entries for each client to reduce the average inference delay for all clients. Assuming each client $k$ has $\mathbf{n}_k$ samples, the average inference latency $\mathcal{T}(\mathbf{W})$ can be defined as:
\begin{equation}
    \mathcal{T}(\mathbf{W}) = \frac{1}{\sum_{k=1}^{\mathbf{N}} \mathbf{n}_k} \cdot \sum_{k=1}^{\mathbf{N}} \mathbf{n}_k \cdot {\mathcal{T}}^{k}(\mathbf{W}^k) 
\end{equation}
where $\mathcal{T}(\mathbf{W})$ represents the global average inference latency and $\mathbf{W}$ is the sum of the parameters of all clients.
We denote the number of samples and the average inference latency at client $k$ as $\mathbf{n}_k$ and ${\mathcal{T}}^{k}(\mathbf{W}^k)$, respectively.
Accordingly, when sample numbers $\mathbf{n}_k$ of each client are consistent, we can define the optimization problem as follows:
$$ \min_{\{\mathbf{W}\}}  \sum_{k=1}^{\mathbf{N}} {\mathcal{T}}^{k}(\mathbf{W}^k) $$ 
\begin{equation}
    s.t. \left\{
    \begin{aligned}
        & \sum_{i \in \mathbf{I}, j \in \mathbf{L}} \mathbf{x}_{i,j}^k \cdot \mathbf{m}_{i,j} \leq \bm{\Pi}^k   \qquad & \forall k  \\
        & \mathcal{G}^k(\mathbf{X}^{k}, \bm{\Theta}^k) \leq \bm{\Omega}^k  \qquad & \forall k  \\
        & \mathbf{x}_{i,j}^k \in \{0, 1\}     \qquad & \forall i,j,k  \\
    \end{aligned}
    \right.
\end{equation}

The object of the optimization problem is to minimize the average inference latency of all clients. The first set of inequalities expresses the cache size constraint for every client, where threshold $\bm{\Pi}^k$ is the cache size threshold prescribed for the client $k$. The second set of inequalities expresses the inference accuracy loss constraints for every client, where threshold $\bm{\Omega}^k$ is the accuracy loss threshold determined for the client $k$. The third set of inequalities represents a reasonable range of values for sign $\mathbf{x}_{i,j}^k$. Equality $\mathbf{x}_{i,j}^k = 1$ means that the cache entry in column $i$, row $j$ of the global cache table is selected for the client $k$, and 0 means the opposite. 
% 填加缓存各列类别相同约束
% 是否添加更多的推导


\subsection{Algorithm Design}

Given the combinatorial explosion, exactly solving this problem is impractical for large instances. Due to our pursuit of low average inference latency, we aim to avoid overly time-consuming allocation algorithms. Therefore, we introduce a cache entry selection algorithm based on a heuristic approach to obtain a suboptimal cache allocation scheme efficiently. We will detail this algorithm in the following sections.

\subsubsection{\textbf{Preliminary Algorithm}} 

Assume that the model has $\mathbf{L}$ cache layers. When making cache entry selection decisions, the server utilizes the class frequency vector $\bm{\Phi}$ and the class timestamp tables $\bm{\tau}^k$ uploaded from the client $k$. Here, $\bm{\Phi}_i$ and $\bm{\tau}_i^k$ represent the values of the class $i$ in each vector, respectively. The global class frequency vector $\bm{\Phi}$ records the occurrence frequency of each class in the inference samples, reflecting the differences in the appearance frequencies of each class. The local class timestamp table $\bm{\tau}$ records the number of consecutive inference samples in which each class has not appeared on the client side, indicating the recency of each class. After each inference, $\bm{\tau}_i^k$ is reset to zero when the sample of class $i$ appears, otherwise incremented by one. $\mathbf{F}$ represents the frequency at which clients update their caches. For every $\mathbf{F}$ inferences, clients initiate cache entry selection requests to the server anew. The client also uploads a cache size constraint threshold $\bm{\Pi}^k$ to guide the selection of cache entries.

% 这一段需要梳理逻辑
The server also receives cache hit ratio vector $\mathbf{R}$ and saved inference time vector $\bm{\Upsilon}$ uploaded by the clients. Both vectors have a length of $\mathbf{L+1}$. The cache hit ratio vector $\mathbf{R}$ records the hit ratio of each cache layer and the saved inference time vector $\bm{\Upsilon}$ records the saved inference time if a cache hit occurs at each cache layer. Combining the contents of these two vectors can help us measure the importance of different cache layers. It assists in retaining more crucial cache entries during cache entry selection.


\subsubsection{\textbf{Algorithm Description}}

\begin{algorithm}[t]
    \caption{Cache Entry Selection} \label{alg:cache select}
    \textbf{Input:}
    \begin{itemize}
        \item Global class occurrence frequency vector $\bm{\Phi}$.
        \item Timestamp vector $\bm{\tau}^k$ received from the client $k$.
        \item hit ratio vector $\mathbf{R}$ and saved inference time vector $\bm{\Upsilon}^k$.
        \item Memory constraint $\bm{\Pi}^k$ for the client $k$.
    \end{itemize}
    \textbf{Output:}
    \begin{itemize}
        \item Selected cache entries indicator table $\mathbf{X}^{k}$ of the client $k$.
    \end{itemize}
    \begin{algorithmic}[1]
        \For {class $i$ in $\mathbf{I}$ classes}
            \State $\mathbf{s}^k_i = \bm{\Phi}_i \cdot (0.20)^{ \lfloor \frac{\bm{\tau}_i^k}{\mathbf{F}} \rfloor }$
        \EndFor
        \State Sort classes in descending order based on their scores ${s}^k$ to obtain the class order list, $\bm{A}$.
        \State $\mathbf{S}^k = 0$ \qquad /* Initialize sum of scores. */
        \State $\mathbf{M}^k = 0$ \qquad /* Initialize sum of size of entries. */
        \For {class $i$ in $\bm{A}$}
            \For {layer $j$ in range($\mathbf{I}$)}
                \State $\mathbf{x}_{i,j}^k = 1$
                \State $\mathbf{M}^k = \mathbf{M}^k + \mathbf{m}_{j}$
            \EndFor
            \State $\mathbf{S}^k = \mathbf{S}^k + \mathbf{s}^k_i$
            \If {$\mathbf{S}^k \geq \sum_{i=1}^I \mathbf{s}^k_i \cdot 95\%$}
                \State Break.
            \EndIf         
        \EndFor
        
        \For {layer $j$ in range($\mathbf{L}$)}
            \State $\bm{\zeta}_{j} = \bm{\Upsilon}_{j}^k \cdot \mathbf{R}_j^k$
        \EndFor
        \State Sort layers in ascending order based on their expected decreased time $\bm{\zeta}$ to obtain the layer order list, $\bm{B}$.
        \For {layer $j$ in $\bm{B}$}
            \If {$\mathbf{M}^k \leq \bm{\Pi}^k$}
                \State Break.
            \Else
                \For {class $i$ in range($\mathbf{I}$)}
                    \State $\mathbf{x}_{i,j}^k = 0$
                \EndFor
                \State $\mathbf{M}^k = \mathbf{M}^k - \mathbf{m}^j \cdot len(\bm{A})$
            \EndIf         
        \EndFor
        \State return $\mathbf{X}^k$.
    \end{algorithmic}
\end{algorithm}

To ensure both cache hit ratio and accuracy, we refer to the method in SMTM. Considering that the class frequency vector and class timestamp vector can represent the frequency and recency of each class, we use the observed data from these two vectors to estimate the probability of each class reoccurring in the future. Specifically, we calculate a score $\mathbf{s}^k_i$ of class $i$ for client $k$ using the following formula:
\begin{equation}
    \mathbf{s}^k_i = \bm{\Phi}_i \cdot (0.20)^{ \lfloor \frac{\bm{\tau}_i^k}{\mathbf{F}} \rfloor }
    \label{eq:classScore}
\end{equation}
where $\bm{\Phi}_i$ represents the global frequency of class $i$, while $\bm{\tau}_i^k$ represents the timestamp for class $i$ on client $k$. $\mathbf{F}$ denotes the number of inferences in a local inference loop. Classes with higher scores have a higher probability of reoccurrence. We then rank the classes based on these scores and select a subset of the top $K$ classes. Following the principles of SMTM, we choose the subset with scores summing up to 95\% of the total score as the candidate cache entry subset. This ensures a high probability of the class of future inference samples belonging to the selected classes appearing in the cache.

% 标记一下，可以再作修改
In addition to pursuing high cache hit ratio and accuracy, we also aim for improved cache efficiency, avoiding excessive lookup costs that could burden the inference process and aligning with the cache size constraints of clients. Therefore, it's essential to assess the importance of different cache layers and remove less crucial caches. $\mathbf{R}$ and $\bm{\Upsilon}$ reflect the probabilities of cache hits at each cache layer and the magnitude of reduced inference latency brought by cache hits. We utilize the observed data from these vectors to estimate the expected latency reduction benefits for each cache layer. Specifically, we calculate the expected reduction benefits by multiplying the corresponding entries in these vectors and then we sort the layers from low to high based on the benefits estimated. Subsequently, we iteratively remove caches from the layers with lower expected benefits until the cache size meets the cache size constraint threshold of the client. This approach ensures that the additional overhead caused by cache lookup is kept within a reasonable range.

% \begin{algorithm}[t]
%     \caption{Cache Entry Selection} \label{alg:cache select}
%     \textbf{Input:}
%     \begin{itemize}
%         \item Global class occurrence frequency vector $\bm{\Phi}$.
%         \item Timestamp vector $\bm{\tau}^k$ received from the client $k$.
%         \item hit ratio vector $\mathbf{R}$ and saved inference time vector $\bm{\Upsilon}^k$.
%         \item Memory constraint $\bm{\Pi}^k$ for the client $k$.
%     \end{itemize}
%     \textbf{Output:}
%     \begin{itemize}
%         \item Selected cache entries indicator table $\mathbf{X}^{k}$ of the client $k$.
%     \end{itemize}
%     \begin{algorithmic}[1]
%         \For {class $i$ in $\mathbf{I}$ classes}
%             \State $\mathbf{s}^k_i = \bm{\Phi}_i \cdot (0.20)^{ \lfloor \frac{\bm{\tau}_i^k}{\mathbf{F}} \rfloor }$
%         \EndFor
%         \State Sort classes in descending order based on their scores ${s}^k$ to obtain the class order list, $\bm{A}$.
%         \State $\mathbf{S}^k = 0$ \qquad /* Initialize sum of scores. */
%         \State $\mathbf{M}^k = 0$ \qquad /* Initialize sum of size of entries. */
%         \For {class $i$ in $\bm{A}$}
%             \For {layer $j$ in range($\mathbf{I}$)}
%                 \State $\mathbf{x}_{i,j}^k = 1$
%                 \State $\mathbf{M}^k = \mathbf{M}^k + \mathbf{m}_{j}$
%             \EndFor
%             \State $\mathbf{S}^k = \mathbf{S}^k + \mathbf{s}^k_i$
%             \If {$\mathbf{S}^k \geq \sum_{i=1}^I \mathbf{s}^k_i \cdot 95\%$}
%                 \State Break.
%             \EndIf         
%         \EndFor
        
%         \For {layer $j$ in range($\mathbf{L}$)}
%             \State $\bm{\zeta}_{j} = \bm{\Upsilon}_{j}^k \cdot \mathbf{R}_j^k$
%         \EndFor
%         \State Sort layers in ascending order based on their expected decreased time $\bm{\zeta}$ to obtain the layer order list, $\bm{B}$.
%         \For {layer $j$ in $\bm{B}$}
%             \If {$\mathbf{M}^k \leq \bm{\Pi}^k$}
%                 \State Break.
%             \Else
%                 \For {class $i$ in range($\mathbf{I}$)}
%                     \State $\mathbf{x}_{i,j}^k = 0$
%                 \EndFor
%                 \State $\mathbf{M}^k = \mathbf{M}^k - \mathbf{m}^j \cdot len(\bm{A})$
%             \EndIf         
%         \EndFor
%         \State return $\mathbf{X}^k$.
%     \end{algorithmic}
% \end{algorithm}

Based on the algorithm design idea mentioned above, we propose a two-stage cache entry selection Algorithm \ref{alg:cache select}. The algorithm takes inputs including global class frequency vector $\bm{\Phi}$ and local class timestamp vector $\bm{\tau}^k$, cache hit ratio vector $\mathbf{R}$, saved inference time vector $\bm{\Upsilon}^k$, and cache size constraint thresholds $\bm{\Pi}^k$. It returns a cache entry selection indicator table $\mathbf{x}^k$ as output. Our proposed algorithm is divided into two stages as follows:
(1) In the first stage, it assesses the importance of each class in the cache and selects hot-spot classes from the row dimension. Initially, it calculates cache class importance scores based on frequency and recency, sorting them in descending order to obtain a ranked list (Lines 1-3). Then, suitable cache class entries are selected and cache sizes are computed (Lines 4-12).
(2) In the second stage, it evaluates the importance of cache layers and removes less crucial cache entries from the column dimension. It measures the importance of each layer based on hit ratio and time savings, sorting them in ascending order to obtain a ranked list (Lines 13-15). Finally, cache entries from less important layers are sequentially removed to meet the cache size threshold constraints of the client (Lines 16-22). The algorithm ultimately returns the generated cache entry selection indicator table (Line 23).

==> his/evaluation6.tex <==

\subsection{Datasets and Models}
\label{subsec:Datasets and Models}

\subsubsection{\textbf{Datasets}}
To validate the effectiveness of our proposed framework COLA, we employ two real-world datasets for classification and recognition tasks respectively.

\begin{itemize}
    \item \textbf{ImageNet-100 \cite{deng2009imagenet}} is a subset of the ImageNet dataset that contains 100 classes, including animals, plants, everyday items, and vehicles. Each class has approximately 1,000 to 1,300 images, totaling around 100,000 images. 
    Our test dataset is organized into batches, with all samples in a batch sharing the same class label. We use this approach to simulate temporal locality.
    
    \item \textbf{UCF101 \cite{soomro2012ucf101}} is an action recognition dataset with 13,320 videos across 101 action classes, collected from YouTube. It covers five major action classes: human-object interactions, body movements, human-human interactions, playing musical instruments, and sports activities. 
    % The dataset is originally at 25 frames per second, and we sample one frame per 5 frames.
\end{itemize}


% % 
% Firstly, following the approaches outlined in \cite{wang2020optimizing, zhao2018federated}, we use the proportion $p$ to quantify the non-IID degree of client data. Specifically, the dataset is divided into groups based on the number of client groups. For each data group, a proportion $p$ of the data is allocated to one corresponding client group, while the remaining data is distributed equally among the other client groups. 
% % Within each client group, the data for each class is evenly distributed among the clients in that group.
% % When the proportion equals the reciprocal of the number of client groups, data samples are uniformly distributed among clients, resulting in IID data.
% Within each client group, the data of each client is IID. 
% If data across different client groups is IID, then data of all clients is IID.
% % 


To simulate different data distributions, several methods are employed to construct appropriate datasets for the clients.
% 
Firstly, following the approaches outlined in \cite{wang2020optimizing, zhao2018federated}, we use the proportion $p$ to quantify the non-IID degree of client data. In defining $p$, to prevent the value of $p$ from being influenced by the number of clients, we use client groups as the basic unit. Each client group has the same number of clients, and the clients within a group have the same data distribution.
Specifically, the dataset is divided into data groups equal to the number of client groups. The samples of each class are divided among these data groups such that each data group contains samples from a distinct subset of classes, with no overlap in classes between data groups. For each data group, a proportion $p$ of the samples of each class are allocated to one corresponding client group, while the remaining samples are distributed equally among the other client groups. If data across different client groups is IID, then the data of all clients is IID.
% 
% To simulate different data distributions, several methods are employed to construct appropriate datasets for the clients.
% % 
% Firstly, following the approaches outlined in \cite{wang2020optimizing, zhao2018federated}, we use the proportion $p$ to quantify the non-IID degree of client data. In defining $p$, to prevent the value of $p$ from being influenced by the number of clients, we use client groups as the basic unit. Each client group has the same number of clients, and the clients within a group have the same data distribution.
% Specifically, the dataset is divided into data groups equal to the number of client groups. For each data group, a proportion $p$ of the samples of each class are allocated to one corresponding client group, while the remaining samples are distributed equally among the other client groups.
% If data across different client groups is IID, then the data of all clients is IID.

% To simulate different data distributions, several methods are employed to construct appropriate datasets for the clients.
% % 
% Firstly, following the approaches outlined in \cite{wang2020optimizing, zhao2018federated}, we use the proportion $p$ to quantify the non-IID degree of client data. 
% Specifically, the dataset is divided into groups based on the number of client groups. For each data group, a proportion $p$ of the data is allocated to one corresponding client group, while the remaining data is distributed equally among the other client groups. 
% Within each client group, the data of each client is IID. 
% If data across different client groups is IID, then data of all clients is IID.
% 

Secondly, for the long-tail distribution, we follow the method used in \cite{cao2019learning}. 
% We denote the sample number of class $i$ as $\mathbf{d}_i$ and use imbalance ratio $\rho$ to denote the ratio between sample sizes of the most frequent and least frequent class, \ie, $\rho = \frac{ \max_{1\leq i\leq I} {\mathbf{d}_i} }{ \min_{1\leq j\leq I}{\mathbf{d}_j}}$ where $I$ is the total number of classes. 
We denote the sample number of class $i$ as $\mathbf{d}_i$. The imbalance ratio $\mathbf{\rho}$ is defined as the ratio between the sample sizes of the most frequent and least frequent classes. Specifically, $\mathbf{\rho} = \frac{ \max{1 \leq i \leq I} {\mathbf{d}i} }{ \min{1 \leq j \leq I}{\mathbf{d}_j}}$, where $I$ is the total number of classes.
Long-tailed imbalance follows an exponential decay in sample sizes across different classes. 
To create a dataset with 50 classes from ImageNet-100 where the top 20\% most frequent classes possess approximately 60\% of the total samples, we set the imbalance ratio $\mathbf{\rho} = 30$.
% 
Finally, we construct a test dataset to simulate scenarios with feature dynamism caused by time. Specifically, videos from 20 subclasses of the UCF101 dataset are manually concatenated in order based on their backgrounds from day to night.

% In addition, 




\subsubsection{\textbf{Models}}
% To comprehensively assess the performance of COLA across varying depths and complexities, we employ four distinct models on the aforementioned datasets.
To comprehensively assess the performance of COLA across various types and depths of neural networks, we employ four distinct models on the aforementioned datasets. 
% Here, depth refers to the number of layers in a model. 
% Generally, deeper models are more complex due to their increased number of layers.

\begin{itemize}
    \item \textbf{VGG16\_BN \cite{sengupta2019going}} consists of 13 convolutional layers using 3$\times$3 convolutional kernels, 2 dense layers, and a softmax output layer. Additionally, the model incorporates batch normalization layers to optimize the training process.
    
    % \item \textbf{ResNet50 \cite{he2016deep}} is composed of a 7$\times$7 convolutional layer, 16 residual blocks, and a fully connected classify layer. Each residual block consists of two 1x1 convolutional layers and one 3$\times$3 convolutional layer, featuring residual connections that skip several layers to alleviate the vanishing gradient problem. The 16 residual blocks are organized into four sections, comprising 3, 4, 6, and 3 residual blocks, respectively.
    \item \textbf{ResNet50 \cite{he2016deep}} is composed of a 7$\times$7 convolutional layer, 16 residual blocks, and a fully connected classify layer. Each residual block consists of 3 different convolutional layers, featuring residual connections that skip several layers to alleviate the vanishing gradient problem. The 16 residual blocks are organized into four sections, comprising 3, 4, 6, and 3 blocks, respectively.
    
    \item \textbf{ResNet101 \cite{lin2021application}} shares a similar backbone structure as ResNet50, but with an increased depth of 101 layers. 
    % In particular, the number of residual blocks in the third section has increased from 6 to 23. 
    In the four sections, the number of residual blocks is distributed as 3, 4, 23, and 3, totaling 33 residual blocks.
    
    \item \textbf{ResNet152 \cite{prabhakaran2021thermal}} boasts an astonishing depth of 152 layers. The number of residual blocks in each of the four sections is distributed as 3, 8, 36, and 3, totaling 50 residual blocks.
\end{itemize}

% \subsubsection{\textbf{Model and Dataset Details}}
% To train the models, we partition the UCF101 dataset using the official "Trainlist01" and "Testlist01" schemes provided by the original paper.

% Table \label{table:models} presents the performance parameters obtained during training and testing. 

% VGG-type models are known for their higher memory consumption due to numerous fully connected layers. In contrast, ResNet models have lower memory usage as they primarily consist of convolutional layers with fewer parameters. PyTorchvision provides pre-trained models on the ImageNet-1k dataset, which can be directly utilized on ImageNet-100.


\subsection{Baselines and Metrics}

\subsubsection{\textbf{Baselines}}
% 为了验证xxx, 为什么取XXX, 为了做哪方面对比，写清楚对比方案是怎么做的
To comprehensively evaluate the performance of COLA, we choose the following four baselines:

\begin{itemize}
    \item \textbf{Edge-Only} represents the conventional edge inference approach where clients perform inference solely on their devices. This baseline helps establish the standard performance metrics without additional acceleration techniques, providing a reference for evaluating the effectiveness of advanced methods.
    
    \item \textbf{LearnedCache} \cite{balasubramanian2021accelerating} is designed to ensure stable memory usage and consistent time consumption by setting multiple intermediate exits in the model. It allows samples to exit early to save inference time. 
    The decision to exit early or not is determined by a separate small model at each exit.
    We introduce this baseline to compare how model-based multi-exit strategies perform against caching-enhanced methods.
    
    \item \textbf{FoggyCache} \cite{guo2018foggycache} demonstrates the potential of client-server frameworks in leveraging caching for inference acceleration. Different from the semantic caching mechanism, FoggyCache uses the modified A-LSH algorithm for organizing cache objects and uses H-kNN for cache lookup before inference. 
    It highlights the effectiveness of server-assisted caching in reducing inference latency. 
    This baseline serves as a comparison object for a different single-exit caching framework in multi-client scenarios.
    
    % \item \textbf{SMTM} \cite{li2021boosting} implements multi-exit inference acceleration using a semantic caching mechanism. It reduces cache space occupancy through compressed cache entry representations. We introduce this baseline to validate the effectiveness of our optimized multi-client cache allocation strategy.
    \item \textbf{SMTM} \cite{li2021boosting} implements multi-exit inference acceleration using a semantic caching mechanism. It reduces cache space occupancy through compressed cache entry representations. We extend its application to multiple clients, using it as a baseline for multi-exit caching in multi-client scenarios.
\end{itemize}


\subsubsection{\textbf{Metrics}}
We adopt the following two metrics to evaluate the performance of COLA and the baselines.

\begin{itemize}
    \item \textbf{Average Latency.} We measure the inference latency for each client on their respective datasets. The total inference time is obtained by summing these values, and the average inference latency is calculated by dividing this sum by the total number of samples.

    \item \textbf{Overall Accuracy.} We define the overall accuracy, which calculates the proportion of correctly inference samples on all clients to the total sample, to evaluate the inference performance of the various acceleration methods. 
\end{itemize}

% 模型的一些训练和内存指标
% \begin{table}[t]
%     \centering
%     \caption{The performance parameters of different CNN models (Accuracy on UCF101 test dataset).}
%     % \vspace{-2mm}
%     \label{table:models}
%     \begin{tabular}{ c | c | c }
%         \hline
%         \rule{0pt}{10pt}
%         Models      &  Memory Size (Mb)  &   Accuracy    \\
%         \hline
%         \rule{0pt}{10pt}
%         VGG16\_BN   &  514  &  78.64    \\  
%         \rule{0pt}{10pt} 
%         ResNet50    &  91   &  80.14    \\  
%         \rule{0pt}{10pt}
%         ResNet101   &  164  &  82.07    \\  
%         \rule{0pt}{10pt}
%         ResNet152   &  224  &  84.32    \\
%     \hline
%     \end{tabular}
%     % \vspace{-0.2cm}
% \end{table}

% \subsection{Experimental Settings}
% \subsubsection{\textbf{Hardware Details}}
% \subsection{Settings Detail}
\subsection{System Implementation}
We utilize the NVIDIA Jetson TX2 \cite{suzen2020benchmark} as our experimental platform to simulate a realistic edge computing environment. The Jetson devices are configured as clients and servers responsible for loading inference models and datasets. The experimental network is established using a router, enabling wireless connections between clients and the server. Our software implementation employs Docker Swarm \cite{singh2023load} for distributed software development and the PyTorch deep learning framework. Docker Swarm facilitates the development of distributed solutions and provides monitoring capabilities for each client's status. The PyTorch deep learning framework enables the efficient execution of complex inference operations on the clients. Moreover, the communication system of the experimental platform is built using Message Passing Interface (MPI) \cite{ragunthar2021strong}, optimizing parallel communication functions through send and receive operations.
% MPI 是否需要插入引用

% parameters setting？

\subsection{Overall Performance}

\begin{table}[t]
\centering
\setlength{\abovecaptionskip}{10pt}%
\setlength{\belowcaptionskip}{0pt}%
\footnotesize
\caption{Inference latency (Late./ms) and accuracy (Acc./\%) on a 50-class subset of the UCF101 dataset within given accuracy constraints. Edge-Only provides the standard latency and accuracy performance used as constraint benchmarks.}
\label{table:Acc cons}
% \begin{tabular}{ cp{0.1\textwidth} cp{0.1\textwidth} cp{0.05\textwidth} cp{0.05\textwidth} cp{0.05\textwidth} cp{0.05\textwidth} }
\begin{tabular}{ c c c c c c }
\hline
\rule{0pt}{8pt}
\multirow{2}{*}{ Models } & \multirow{2}{*}{ Methods } & \multicolumn{2}{c}{<3\%} & \multicolumn{2}{c}{<5\%} \\
\cline{3-6}
\rule{0pt}{8pt}
 &  & Late. & Acc. & Late. & Acc. \\
\hline
\rule{0pt}{8pt}
\multirow{5}{*}{VGG16\_BN} & Edge-Only           &  29.94 & 78.12 & 29.94 & 78.12   \\
\cline{2-6}
\rule{0pt}{8pt}
& LearnedCache & 26.82 & 75.28 & 23.98 & 73.86 \\
\cline{2-6}
\rule{0pt}{8pt}
& FoggyCache & 27.12 & 75.37 & 23.42 & 73.89 \\
\cline{2-6}
\rule{0pt}{8pt}
& SMTM & 25.51  & 75.41 & 22.15  & 73.97   \\
\cline{2-6}
\rule{0pt}{8pt}
& \textbf{COLA} & \textbf{23.05} & {75.73} & \textbf{20.36} & {74.23}  \\
\hline
\rule{0pt}{8pt}
\multirow{5}{*}{ResNet50} & Edge-Only              & 29.56 & 80.23 & 29.56 & 80.23 \\
\cline{2-6}
\rule{0pt}{8pt}
& LearnedCache & 26.94 & 77.73 & 23.96 & 75.56 \\
\cline{2-6}
\rule{0pt}{8pt}
& FoggyCache & 27.29 & 77.68 & 22.77 & 75.76 \\
\cline{2-6}
\rule{0pt}{8pt}
& SMTM & 25.12  &  77.59  & 22.13  & 75.83   \\
\cline{2-6}
\rule{0pt}{8pt}
& \textbf{COLA} & \textbf{22.46} & {78.16} & \textbf{19.80} & {76.38}  \\
\hline
\rule{0pt}{8pt}
\multirow{5}{*}{ResNet101} & Edge-Only             & 44.92 & 82.71 & 44.92 & 82.71 \\
\cline{2-6}
\rule{0pt}{8pt}
& LearnedCache & 35.93 & 80.62 & 33.69   & 77.94 \\
\cline{2-6}
\rule{0pt}{8pt}
& FoggyCache & 34.76 & 80.92 & 31.62 & 78.11 \\
\cline{2-6}
\rule{0pt}{8pt}
& SMTM & 33.95  & 80.76   & 29.46  & 78.20   \\
\cline{2-6}
\rule{0pt}{8pt}
& \textbf{COLA} & \textbf{28.29} & {81.05} & \textbf{24.26} & {78.94}  \\
\hline
\rule{0pt}{8pt}
\multirow{5}{*}{ResNet152} & Edge-Only              & 62.85 & 83.98 & 62.85 & 83.98 \\
\cline{2-6}
\rule{0pt}{8pt}
& LearnedCache & 48.39 & 81.30 & 43.74 & 79.31 \\
\cline{2-6}
\rule{0pt}{8pt}
& FoggyCache & 45.22 & 81.63 & 39.69 & 79.51 \\
\cline{2-6}
\rule{0pt}{8pt}
& SMTM & 44.83  & 81.72 & 35.54  & 79.46   \\
\cline{2-6}
\rule{0pt}{8pt}
& \textbf{COLA} & \textbf{34.45} & {82.16} & \textbf{29.53} & {79.82}  \\
\hline
\end{tabular}
\end{table}

                                         


\subsubsection{\textbf{Latency reduction within accuracy constraints}}

% 
We conduct experiments on the UCF101 datasets to evaluate the average inference latency of COLA and various baselines with specific accuracy loss constraints (\eg, 3\% and 5\%). 
Table \ref{table:Acc cons} presents the test results on a subset of 50 classes from UCF101.
% result
As shown in the table, COLA consistently achieves greater latency reductions within the given accuracy loss constraints compared to the baselines. For instance, under a 3\% accuracy loss constraint, COLA reduces the average inference latency by 23.01\%, 24.02\%, 37.02\%, and 45.19\% on VGG16\_BN, ResNet50, ResNet101, and ResNet152 respectively, compared to Edge-Only. 
Specifically, COLA achieves latency reductions of 16.67\%-21.26\% on the ResNet101 model compared to other acceleration baselines.
% conclusion and reason 
Unlike traditional multi-exit methods, COLA employs semantic caching to reduce computational overhead, resulting in improved latency reductions. Compared to SMTM, COLA utilizes a more granular dynamic local cache allocation, better balancing accuracy and latency performance and achieving lower average inference latency.
% 
In summary, COLA demonstrates significant improvements in inference latency across different models and datasets, showing its potential as an effective acceleration framework.


\begin{table}[t]
\centering
\setlength{\abovecaptionskip}{10pt}%
\setlength{\belowcaptionskip}{0pt}%
\footnotesize
\caption{Inference accuracy (Acc./\%) and latency (Late./ms)  within given latency reduction targets. Edge-Only provides the standard latency and accuracy performance used as constraint benchmarks.}
\label{table:Late cons}
% \begin{tabular}{ cp{0.1\textwidth} cp{0.1\textwidth} cp{0.05\textwidth} cp{0.05\textwidth} cp{0.05\textwidth} cp{0.05\textwidth} }
\begin{tabular}{ c c c c c c }
\hline
\rule{0pt}{8pt}
\multirow{2}{*}{ Models } & \multirow{2}{*}{ Methods } & \multicolumn{2}{c}{$\geq$ 15\%} &  \multicolumn{2}{c}{$\geq$ 30\%} \\
\cline{3-6}
\rule{0pt}{8pt}
 &  & Acc. & Late. & Acc. & Late. \\
\hline
\rule{0pt}{8pt}
\multirow{5}{*}{VGG16\_BN} & Edge-Only          & 78.12 &  100.0 & 78.12 & 100.0    \\
\cline{2-6}
\rule{0pt}{8pt}
& LearnedCache & 74.25 & 83.73 & 66.10 & 69.64 \\
\cline{2-6}
\rule{0pt}{8pt}
& FoggyCache & 74.27 & 83.24 & 67.43 & 69.45 \\
\cline{2-6}
\rule{0pt}{8pt}
& SMTM & 75.07  & 84.61 & 70.68  & 69.48   \\
\cline{2-6}
\rule{0pt}{8pt}
& \textbf{COLA} & \textbf{76.61} & 84.90 & \textbf{74.23} & 68.00  \\
\hline
\rule{0pt}{8pt}
\multirow{5}{*}{ResNet50} & Edge-Only             & 80.23 & 100.0 & 80.23 & 100.0 \\
\cline{2-6}
\rule{0pt}{8pt}
& LearnedCache & 75.82 & 83.90 &  62.29 & 68.20 \\
\cline{2-6}
\rule{0pt}{8pt}
& FoggyCache & 76.16 & 83.31 & 67.40 & 67.58 \\
\cline{2-6}
\rule{0pt}{8pt}
& SMTM & 77.59  & 84.98   & 71.04  & 69.09   \\
\cline{2-6}
\rule{0pt}{8pt}
& \textbf{COLA} & \textbf{78.47} & 80.18 & \textbf{76.38} & 66.98  \\
\hline
\rule{0pt}{8pt}
\multirow{5}{*}{ResNet101} & Edge-Only            & 82.71 & 100.0 & 82.71 & 100.0 \\
\cline{2-6}
\rule{0pt}{8pt}
& LearnedCache & 80.71 & 80.21 & 77.45 & 68.96  \\
\cline{2-6}
\rule{0pt}{8pt}
& FoggyCache & 81.07 & 80.77 & 78.02 & 69.15 \\
\cline{2-6}
\rule{0pt}{8pt}
& SMTM & 81.11  & 81.55  & 79.20  &  65.58  \\
\cline{2-6}
\rule{0pt}{8pt}
& \textbf{COLA} & \textbf{81.88} & 81.82 & \textbf{81.05} & 62.98  \\
\hline
\rule{0pt}{8pt}
\multirow{5}{*}{ResNet152} & Edge-Only             & 83.98 & 100.0 & 83.98 & 100.0 \\
\cline{2-6}
\rule{0pt}{8pt}
& LearnedCache & 81.67 & 80.55 &  79.31 & 69.59 \\
\cline{2-6}
\rule{0pt}{8pt}
& FoggyCache & 82.39 & 83.77 & 81.14 & 68.94 \\
\cline{2-6}
\rule{0pt}{8pt}
& SMTM & 82.47  & 81.06   & 81.43  & 68.37   \\
\cline{2-6}
\rule{0pt}{8pt}
& \textbf{COLA} & \textbf{83.21} & 80.58 & \textbf{82.51} & 65.31  \\
\hline
\end{tabular}
\end{table}

 

\subsubsection{\textbf{Maintaining accuracy with latency reduction targets}}
% 可以尝试更加简练
% Then, we evaluate the accuracy loss of COLA and the baselines under different inference latency reduction targets (\eg, 15\% and 30\%).
We evaluate the accuracy loss of COLA and the baselines under different relative inference latency reduction targets (\eg, 15\% and 30\% compared to the Edge-Only baseline).
% result
As shown in Table \ref{table:Late cons}, COLA consistently incurs lower inference accuracy loss compared to other acceleration baselines while achieving the specified average latency reduction targets. 
Notably, when achieving the 15\% average latency reduction target, COLA incurs an accuracy loss of 0.83\% and 0.77\% on the ResNet101 and ResNet152 models, respectively. 
In contrast, other baselines generally exhibit accuracy losses exceeding 1\%.
% conclusion and reason
COLA and SMTM generally outperform LearnedCache and FoggyCache regarding accuracy. When relaxing exit conditions to achieve latency reduction targets, LearnedCache and FoggyCache suffer higher accuracy losses. For instance, exit models of LearnedCache are more prone to misclassifications. 
Under looser exit conditions, cache hits are more likely to happen at shallow cache layers during inference for SMTM, leading to an increased error ratio. In contrast, COLA meticulously selects cache layers, thereby achieving superior inference accuracy compared to SMTM.
These results demonstrate that COLA can significantly reduce the average inference latency while incurring slight inference accuracy loss.


\subsection{The Effect of Imbalanced Data}
% 长尾分布和数据特性变化 放在这 
We investigate the performance of COLA regarding imbalanced data distributions. 
Under this situation, we mainly consider long-tail distributions and non-IID cases. 
First, for the long-tail distribution, we established two groups: one with a uniform distribution across classes (uniform group) and the other following a long-tail distribution (long-tail group), based on a subset of 50 classes from ImageNet-100.
The long-tail distribution is created as described in Section \ref{subsec:Datasets and Models}, resulting in approximately 60\% of the data belonging to the top 20\% frequent classes.
% results
We repeatedly test the inference latency and accuracy of COLA and baselines on these two groups 5 times and report the average results, as shown in Table \ref{table:longtail}. 
LearnedCache and FoggyCache perform similarly across uniform and long-tail groups. COLA and SMTM exhibit significantly lower inference latency for the long-tail group compared to the uniform group. 
COLA outperforms all baselines in both groups, achieving the lowest latency while maintaining competitive accuracy. Specially, COLA reduces inference latency by 4.01\% in the long-tail group compared to the uniform group, while maintaining an accuracy of 81.35\%.
% reason and conclusion
% This can be attributed to two factors: firstly, the higher proportion of frequent classes in the long-tail group setup leads to an increased cache hit ratio. secondly, the cache allocation strategy of COLA handles long-tail distributions more effectively compared to the simple LRU strategy.
This can be attributed to two factors. 
Firstly, the higher proportion of frequent classes in the long-tail group indirectly enhances temporal locality within the dataset, thereby resulting in an increased cache hit ratio. 
Secondly, the cache allocation strategy of COLA handles long-tail distributions more effectively compared to the simple LRU strategy.
In summary, by adapting to data distribution and optimizing cache allocation, COLA significantly reduces latency while maintaining accuracy, which suggests the potential benefits of COLA in real-world scenarios with long-tail data distributions.


\begin{figure*}[t]
    \newcounter{tempfigcnt}
    \setcounter{tempfigcnt}{\value{figure}}
    \vspace{-3mm}
    \includegraphics[width=\textwidth]{fig/Latency_Legends.pdf}
    \vspace{-4mm}
    \label{late-legend}
    \addtocounter{figure}{-1}\setcounter{figure}{\value{tempfigcnt}}
\end{figure*}

\begin{figure*}[t]
    \vspace{-3mm}
    \includegraphics[width=\textwidth]{fig/Latency.pdf}
    \vspace{-4mm}
    \caption{Latency performance of COLA and baselines on UCF and ImageNet at different non-IID degrees across different models.}
    \label{fig:NonIID-late}
\end{figure*}

\begin{figure*}[t]
    \setcounter{tempfigcnt}{\value{figure}}
    \vspace{-3mm}
    \includegraphics[width=\textwidth]{fig/Accuracy_Legends.pdf}
    \vspace{-4mm}
    \label{acc-legend}
    \addtocounter{figure}{-1}\setcounter{figure}{\value{tempfigcnt}}
\end{figure*}

\begin{figure*}[t]
    \vspace{-3mm}
    \includegraphics[width=\textwidth]{fig/Accuracy.pdf}
    \vspace{-4mm}
    \caption{Accuracy performance of COLA and baselines on UCF and ImageNet at different non-IID degrees across different models.}
    \label{fig:NonIID-acc}
\end{figure*}


Second, to assess the performance of COLA on non-IID data, we conduct experiments on ImageNet-100 and a subset of 50 classes from UCF101 with varying non-IID degrees ($p=0.25, 0.5, 0.7, 0.9$), and the test results are shown in 
Figs. \ref{fig:NonIID-late} and \ref{fig:NonIID-acc}.
% results
On the one hand, the methods without caching demonstrate stable average inference latency and accuracy performance across different non-IID degrees. For instance, the relative difference in average inference latency of Edge-Only on the ResNet152 model remains within 1\% across various non-IID degrees.
% , indicating high stability. 
In contrast, caching-based methods exhibit a trend of decreasing average inference latency and increasing accuracy as the non-IID degree rises.
COLA shows a consistent reduction in average inference latency across all clients as the non-IID degree increases. Specifically, under the highest non-IID degree ($p=0.9$), the average latency of ResNet101 decreases by approximately 9.08\% compared to the IID case ($p=0.25$). This reduction is more significant than that with FoggyCache and SMTM.
Simultaneously, the inference accuracy of COLA steadily improves, with the accuracy loss decreasing from nearly 3\% (under IID) to less than 1\% at non-IID degree $p=0.9$.

On the other hand, COLA consistently outperforms acceleration baselines in both latency reduction across the different models and non-IID degrees. For the ResNet101 model, COLA achieves a 36.97\%-42.88\% reduction in latency compared to Edge-Only and an additional 17.96\%-21.04\% reduction compared to SMTM, under the different non-IID degrees.
% reason and conclusion
%These results align with our predictions. 
As the non-IID degree of the data increases, temporal locality becomes more pronounced, enhancing the effectiveness of cache-based methods like COLA. This leads to an improved likelihood and accuracy of cache hits, ultimately reducing average inference latency and minimizing inference accuracy loss. Among these methods, COLA performs particularly well with increased non-IID degrees. This superior performance is primarily due to global updates, which enhance the representativeness of global cache entries, thereby improving both cache hit ratio and inference accuracy.
In summary, the experimental results demonstrate that COLA not only significantly reduces average inference latency but also maintains higher inference accuracy compared to other baseline methods, which underscores the robustness and effectiveness of COLA, particularly in scenarios with high non-IID data distributions.

% Finally, to evaluate the performance of COLA in scenarios with feature dynamism, a test dataset simulating the passage of time is constructed. Specifically, videos from 20 subclasses of the UCF101 dataset are manually selected and concatenated following a pattern from day to night. 
% The inference latency and accuracy of COLA with and without global updating, as well as baseline methods, are tested on this dataset, with the results shown in the table. Compared to not using global updates, COLA with global updates achieves an additional 2.54\% reduction in inference latency and a 0.45\% improvement in accuracy. The accuracy improvement primarily stems from global updates maintaining the representativeness of the cache for the features of the inference samples, thereby making the semantic center directions of different classes more representative.


% \begin{table}[t]
% \centering
% \setlength{\abovecaptionskip}{10pt}%
% \setlength{\belowcaptionskip}{0pt}%
% \footnotesize
% \caption{The average inference latency (Late.) and accuracy (Acc.) of ResNet101 on the constructed streaming UCF dataset with and without global updates.}
% \label{table:time}
% \begin{tabular}{ c c c }
% \hline
% \rule{0pt}{8pt}
%                     & Late. & Acc. \\
% \hline
% \rule{0pt}{8pt}
% Edge-Only              & 44.95 & 82.82    \\
% \hline
% \rule{0pt}{8pt}
% LearnedCache            & 35.98 & 80.67   \\
% \hline
% \rule{0pt}{8pt}
% FoggyCache          & 34.85 & 80.93  \\
% \hline
% \rule{0pt}{8pt}
% COLA (without)      & 28.97 & 80.78 \\
% \hline
% \rule{0pt}{8pt}
% COLA (with)         & 27.63 & 81.23  \\
% \hline
% \end{tabular}
% \end{table}


\begin{table}[t]
\centering
\setlength{\abovecaptionskip}{10pt}%
\setlength{\belowcaptionskip}{0pt}%
\footnotesize
\caption{The average inference latency (Late./ms) and accuracy (Acc./\%) of ResNet101 on constructed uniformed and long-tail groups dataset of ImageNet-100.}
\label{table:longtail}
\begin{tabular}{ c c c c c}
\hline
\rule{0pt}{8pt}
            & \multicolumn{2}{c}{uniformed} &  \multicolumn{2}{c}{long-tail} \\
\cline{2-5}
\rule{0pt}{8pt}
            & Late. & Acc. & Late. & Acc. \\
\hline
\rule{0pt}{8pt}
Edge-Only      & 44.87 & 82.64  & 44.91  &  82.67   \\
\hline
\rule{0pt}{8pt}
LearnedCache    & 35.81 & 80.56  & 36.02  &  80.61   \\
\hline
\rule{0pt}{8pt}
FoggyCache  & 34.64 & 80.83  & 34.83  & 80.88    \\
\hline
\rule{0pt}{8pt}
SMTM        & 34.02 & 80.68  & 33.29  & 80.92    \\
\hline
\rule{0pt}{8pt}
COLA        & 28.17 & 80.97  & 27.04  & 81.35    \\
\hline
\end{tabular}
\end{table}


\subsection{The Effect of Model Size}

From the previous experimental results, COLA performs better on complex models compared to simpler ones. To further investigate the relationship between model size and the effectiveness of COLA, we test the performance of ResNet50, ResNet101, and ResNet152 models on a subset of 50 classes from UCF101 with IID distribution. We compare their performance under 3\% and 5\% accuracy loss constraints. By analyzing the differences in latency reduction effects between COLA and the baselines, we aim to provide a deeper understanding of how model size influences the latency reduction capabilities of these methods.

% results
In Fig. \ref{fig:Serial}, COLA consistently outperforms the baselines in terms of average inference latency reduction, regardless of the model or accuracy loss constraint. Under a 5\% accuracy loss, COLA achieves a 33\%-61\% reduction in average inference latency, significantly surpassing the 25\%-43\% reduction of SMTM. This demonstrates the superior ability of COLA to achieve lower average latency compared to baselines, even for models with varying complexities.
% reason
Furthermore, under a 3\% accuracy loss constraint, the advantage of COLA becomes more pronounced as model size and complexity increase. Specifically, we observe latency reductions of 24.02\%, 37.02\%, and 45.19\% for ResNet50, ResNet101, and ResNet152, respectively, compared to Edge-Only. This trend can be attributed to the inherent increase in inference latency as model complexity grows, while the computation of cache lookup remains relatively minor and does not introduce significant lookup time. Besides, as model complexity increases, the number of cache layers also increases. A larger global cache table amplifies the advantages of COLA's cache allocation algorithm. The latency reduction of the early exit mechanism becomes more pronounced as the model size increases, leading to greater latency reductions.
% conclusion
These findings demonstrate the effectiveness of COLA in accelerating inference across models of varying complexities, with the advantages becoming more pronounced for larger and more complex models. 
% This can be partly explained by the increasing significance of early exit as the model size grows, which COLA leverages to achieve superior latency reduction.

\begin{figure}[t]
  \centering
  \hspace{-2.5mm}\subfigure[3\% of Accuracy]{\includegraphics[width=1.625in]{fig/3-Serial-Models-Fig.pdf}}
  \hspace{4.5mm}
  \subfigure[5\% of Accuracy]{\includegraphics[width=1.625in]{fig/5-Serial-Models-Fig.pdf}}
  \caption{Latency performance across different models with accuracy constraints.}
  \label{fig:Serial}
\end{figure}


% \subsection{The Effect of Global Updates}
% 本小节直接并入消融实验部分，作为一个小节

% \begin{figure}[t]
%   \centering
%   \hspace{-5mm}\subfigure[ResNet101]{\includegraphics[width=1.7in]{fig/DataEffect-ResNet101.pdf}}
%   \hspace{2.5mm}
%   \subfigure[VGG16\_BN]{\includegraphics[width=1.7in]{fig/DataEffect-Vgg16_bn.pdf}}
%   \caption{The trend of the accuracy of the inference with (w.) and without (wo.) global updates as data volume increases across different models.}
%   \label{fig:Update}
% \end{figure}


% In COLA, the global cache is updated using the data collected from clients during the inference process. To investigate the impact of global cache updates on inference accuracy, comparative experiments with and without global cache updates were conducted on the ResNet101 and VGG16\_BN models.
% The control group consistently utilizes cache pre-generated by the cloud using a public dataset, while the experimental group collects information during the inference process and updates the cloud cache accordingly. Fig. \ref{fig:Update} illustrates how the accuracy of both approaches changes with increasing amounts of inference data.

% For the ResNet101 model, the results show noticeable fluctuations in the accuracy of both approaches during the first 2,000 images. However, the overall trend for both groups exhibits an upward trajectory thereafter. Notably, after reaching the 4,000-th image, the experimental group's accuracy performance starts to significantly surpass that of the control group, and this advantage continues until around 18000 images. In the final measurement (at the 17,687-th image), the experimental group achieves an accuracy of 81.80\%, while the control group achieves 80.52\%, resulting in a 1.28\% higher accuracy for the experimental group. For the VGG16\_BN model, the experimental results also exhibit a similar trend, with the accuracy finally differing by around 1.74\% between employing the global updating strategy and not using this strategy.

% These findings suggest that the experimental group, which adopts the global cache updates, achieves a notable improvement in accuracy compared to the control group. This can be attributed to the benefits of leveraging the continuously updated cache, which likely captures the evolving characteristics of the inference data more effectively than the static cache used by the control group.


\subsection{Ablation Study}


To investigate the specific effects of the two main components of COLA, \ie, dynamic cache allocation and global cache updates, on average inference latency and accuracy, we conduct the following ablation experiments.
Four approaches are compared in terms of their performance: Normal (standard), DCA (dynamic cache allocation only), GCU (global cache updates only), and DCA+GCU (utilizing both two components).
% 
The results in Fig. \ref{fig:Ablation} indicate that employing both improvements simultaneously (\ie, DCA+GCU) yields superior performance in terms of average inference latency and accuracy compared to utilizing either improvement alone (DCA or GCU).
% % Latency Reduction
% The DCA results in a more significant latency reduction across all four models compared to the GCU. For instance, on the ResNet152 model, the GCU achieves a 6.6\% latency reduction relative to Normal, while DCA achieves a remarkable 39.2\% reduction, leading GCU by 32.6\%. This suggests that the dynamic cache allocation in the DCA plays a dominant role in latency reduction, as it directly impacts the cache lookup overhead and hit ratio. In contrast, the GCU indirectly improves inference by utilizing more representative cache entries, resulting in a relatively smaller impact.
% % Accuracy Improvement
% In terms of accuracy performance, the GCU exhibits relatively lower accuracy loss across all four models compared to the DCA. For the ResNet101 model, the accuracy loss of DCA relative to Normal is 2.01\%, while GCU achieves an accuracy loss of only 1.49\%, a reduction of 0.52\% or nearly 25\%. The combination of both improvements (DCA+GCU) results in the best accuracy performance, likely due to the combinational effects that GCU enhances the representativeness of cache entries for DCA while DCA provides better cache management to avoid excessive interference from redundant cache entries.
% Latency Reduction
The DCA can achieve a more significant latency reduction across all four models compared to the GCU. 
For instance, we compare the performance of different methods on the ResNet152 model, using Normal as the baseline. The results show that GCU achieves a 6.60\% latency reduction. In contrast, DCA demonstrates superior performance with a remarkable 39.18\% reduction in latency. 
In other words, DCA outperforms GCU by a significant margin of 32.58\% in latency reduction, which suggests that DCA plays a dominant role in latency reduction, as it directly impacts the cache lookup overhead and hit ratio. In contrast, GCU indirectly improves the cache hit ratio by utilizing more representative cache entries, resulting in a relatively smaller impact.
% Accuracy Improvement
In terms of accuracy performance, GCU exhibits relatively lower accuracy loss across all four models compared to DCA. For the ResNet101 model, the accuracy loss of DCA relative to Normal is 2.01\%, while GCU achieves an accuracy loss of only 1.49\%, a reduction of 0.52\%, or nearly 25\%. 
The combination of both components (\ie, DCA+GCU) results in the best accuracy performance. This is likely due to the combinational effects where GCU enhances the representativeness of cache entries for DCA, while DCA provides better cache management to avoid excessive interference from redundant cache entries.
The above findings demonstrate the complementary nature of the two key components of COLA and the importance of their joint application to achieve optimal performance in terms of both latency reduction and accuracy maintenance.

% 添加 全局更新部分更详细的描述
% \begin{figure}[t]
%   \centering
%   \hspace{-5mm}\subfigure[ResNet101]{\includegraphics[width=1.7in]{fig/DataEffect-ResNet101.pdf}}
%   \hspace{2.5mm}
%   \subfigure[VGG16\_BN]{\includegraphics[width=1.7in]{fig/DataEffect-Vgg16_bn.pdf}}
%   \caption{The trend of the accuracy of the inference with (w.) and without (wo.) global updates as data volume increases across different models.}
%   \label{fig:Update}
% \end{figure}

% In COLA, the global cache is updated using the data collected from clients during the inference process. 
% To further investigate the impact of global cache updates on inference accuracy, we conduct comparative experiments with and without global cache updates on the ResNet101 and VGG16\_BN models.
% The control group consistently utilizes cache pre-generated by the cloud using a public dataset, while the experimental group collects information during the inference process and updates the global cache. Fig. \ref{fig:Update} illustrates how the accuracy of both approaches changes with increasing amounts of inference data.
% % 
% For the ResNet101 model, the results show noticeable fluctuations in the accuracy of both approaches during the first 2,000 images. However, the overall trend for both groups exhibits an upward trajectory thereafter. Notably, after reaching the 4,000-th image, the accuracy performance of experimental group starts to significantly surpass that of the control group, and this advantage continues until around 18,000 images. In the final measurement (at the 17,687-th image), the experimental group achieves an accuracy of 81.80\%, while the control group achieves 80.52\%, resulting in a 1.28\% higher accuracy for the experimental group. For the VGG16\_BN model, the experimental results also exhibit a similar trend, with the accuracy finally differing by around 1.74\% between employing the global updating strategy and not using this strategy.
% % 
% These results suggest that the experimental group, which adopts the global cache updates, achieves a notable improvement in accuracy compared to the control group. This can be attributed to the benefits of leveraging the continuously updated cache, which likely captures the evolving characteristics of the inference data more effectively than the static cache used by the control group.
% 
% To further investigate the impact of global cache updates on inference accuracy, we conduct comparative experiments with and without global cache updates on the ResNet101 and VGG16\_BN models. The control group consistently uses a cache pre-generated by the cloud using a public dataset, while the experimental group updates the global cache based on information collected during inference. Fig. \ref{fig:Update} illustrates how the accuracy of both approaches changes with increasing amounts of inference data.
% % 
% For ResNet101, both groups show noticeable fluctuations in accuracy during the first 2,000 images. However, the overall trend for both groups is upward. Notably, after 4,000 images, the accuracy of the experimental group starts to significantly surpass that of the control group, maintaining this advantage until around 18,000 images. In the final measurement (at the 17,687th image), the experimental group achieves an accuracy of 81.80\%, while the control group achieves 80.52\%, resulting in a 1.28\% higher accuracy for the experimental group. For the VGG16\_BN model, a similar trend is observed, with the experimental group showing an accuracy improvement of about 1.74\% over the control group.
% % 
% These results suggest that the experimental group, which adopts global cache updates, achieves a notable improvement in accuracy compared to the control group. This improvement can be attributed to the benefits of continuously updating the cache, which better captures the evolving characteristics of the inference data than the static cache used by the control group.
% % end

% These findings demonstrate the complementary nature of the two key components of COLA and the importance of their joint application to achieve optimal performance in terms of both latency reduction and accuracy maintenance.

% To further investigate the impact of global cache updates on inference accuracy, we conduct comparative experiments with and without global cache updates on the ResNet101 and VGG16\_BN models. The experimental group updates the global cache based on information collected during inference, while the control group consistently uses a cache pre-generated by the cloud using a public dataset. Fig. \ref{fig:Update} illustrates how the accuracy of both approaches changes with increasing amounts of inference data.
% % 
% For ResNet101, both groups show noticeable fluctuations in accuracy during the first 2,000 images. However, the overall trend for both groups is upward. Notably, after 4,000 images, the accuracy of the experimental group starts to significantly surpass that of the control group, maintaining this advantage until around 18,000 images. In the final measurement (at the 17,687th image), the experimental group achieves an accuracy of 81.80\%, while the control group achieves 80.52\%, resulting in a 1.28\% higher accuracy for the experimental group. For the VGG16\_BN model, we observe a similar trend, \ie, the experimental group shows an accuracy improvement of about 1.74\% over the control group.
% % 
% These results suggest that the experimental group, which adopts global cache updates, achieves a notable improvement in accuracy compared to the control group. This improvement can be attributed to the benefits of continuously updating the cache, which better captures the evolving feature of the inference data than the static cache used by the control group.
% The above findings demonstrate the complementary nature of the two key components of COLA and the importance of their joint application to achieve optimal performance in terms of both latency reduction and accuracy maintenance.

\begin{figure}[t]
  \vspace{1.9mm}\centering
  \subfigure[Latency]{\includegraphics[width=1.7in]{fig/Ablation-latency.pdf}}
  %\hspace{2.5mm}
  \subfigure[Accuracy]{\includegraphics[width=1.7in]{fig/Ablation-acc.pdf}}
  \caption{Latency and accuracy performance on 50-class subset of the UCF101 dataset across different models in ablation experiments.}
  \label{fig:Ablation}
\end{figure}


\subsection{Scalability Experiment}


% \begin{figure}[t]
%   \centering
%   \subfigure[Impact of client number on average inference latency.]{\includegraphics[width=1.5in]{fig/Client_num_effect.pdf}}
%   \hspace{2mm}
%   \subfigure[Average inference Latency and accuracy on different frames per cycle.]{\includegraphics[width=1.8in]{fig/Frames_num_effect.pdf}}
%   \caption{Experiments on the effect of the number of clients and frames per cycle.}
%   \label{fig:Scale}
% \end{figure}


\begin{figure}[t]
  \centering
  \subfigure[Average inference Latency and accuracy on different frames per cycle.]{\includegraphics[width=1.9in]{fig/Frames_num_effect.pdf}}
  % \hspace{2mm}
  \subfigure[Impact of client number on average inference latency.]{\includegraphics[width=1.6in]{fig/Client_num_effect.pdf}}
  \caption{Experiments on the effect of the number of clients and frames per cycle.}
  \label{fig:Scale}
\end{figure}



In the previous subsection, we observed the positive impact of global updates and cache allocation on inference accuracy and average latency. In COLA, local clients send global update and cache allocation requests to the server after processing every $\mathbf{F}$ frames. More frequent updates can enhance inference accuracy but may also increase server load, thereby affecting latency performance. To study the impact of $\mathbf{F}$ on inference latency and accuracy, we tested the VGG16\_BN on a dataset containing 50 classes from UCF101. The results are shown in Figure \ref{fig:Scale}(a).

As $\mathbf{F}$ increases, the average inference latency initially decreases significantly. It slows down the decreasing rate and eventually stabilizes when $\mathbf{F}$ is beyond 300. The latency decreases from 45.74 ms at $\mathbf{F}=150$ to 45.02 ms at $\mathbf{F}=900$. Inference accuracy follows a similar decreasing trend. 
The initial significant decrease and subsequent stabilization of latency are primarily due to the reduced impact of server-side time overhead. 
When $\mathbf{F}$ is small, multiple clients are more likely to simultaneously send requests to the server, causing waiting times and increasing server-side time overhead. 
As $\mathbf{F}$ increases, the timeliness of the cache decreases. Furthermore, we use Eq. \ref{eq:classScore} to evaluate the importance of different classes during cache allocation. 
A large $\mathbf{F}$ affects our ability to distinguish the recency of different classes, thereby impacting the effectiveness of cache allocation and resulting in overall decreased inference accuracy.
Balancing accuracy loss and latency reduction, we find that a setting of $\mathbf{F}=300$ is more appropriate. Further increasing $\mathbf{F}$ results in accuracy losses that outweigh the benefits of reduced latency. 
% The optimal $\mathbf{F}$ value depends on the characteristics of the dataset.

COLA employs a multi-client collaborative caching mechanism. 
Under a fixed $F$, the frequency of client requests to the server remains relatively stable. 
In this scenario, the number of clients affects the response rate to requests of the server, thereby impacting the inference performance of the clients.
To explore the scalability of COLA, we investigate the impact of the number of clients on the average inference latency of different models under the setting of $\mathbf{F}=300$. This experiment uses a dataset containing 50 classes from UCF101. The results are shown in Fig. \ref{fig:Scale}(b).
As the number of clients increases, the average inference latency for various models shows an upward trend. For example, in the ResNet101 model, the average inference latency increases from 45.27 ms with 20 clients to 45.83 ms with 100 clients, representing a relative increase of 1.24\%. For the ResNet152 model, the average inference latency with 100 clients rises by 2.58\% compared to the latency with 20 clients. 
The latency reduction effects of COLA remain stable within 100 clients.
With a higher number of clients, the latency performance degrades. 
This is primarily due to the competition for global cache access during asynchronous processing. Each client's cache allocation requests and global updates contend for read and write operations on the global cache. As the number of clients increases, the probability of request collisions at the server side also rises, causing clients to wait for server responses, ultimately leading to an increase in average inference latency.

These results are acceptable. On the one hand, some simple edge systems do not require many clients. For instance, in an industrial pipeline sorting system within a factory \cite{}, a few dozen edge clients can meet the demand. On the other hand, COLA can be extended to accommodate more clients using a simple hierarchical tree structure. In this setup, lower-tier edge servers handle inference acceleration for dozens of clients. These lower-tier servers, in turn, act as clients to an upper-tier server. The upper-tier server periodically updates the caches maintained by the lower-tier servers, enabling the sharing of inference information across a larger number of clients. Furthermore, the operations of the upper-tier server are relatively independent of the lower-tier servers, ensuring that the extension does not directly and significantly impact the inference latency performance of each client.
We implement a simple demo to validate the effectiveness of COLA, with extended version tests planned for future investigation. 



% To enhance the scalability of COLA, various methods can be employed. One straightforward approach is to increase the number of frames per cycle, denoted as $\mathbf{F}$. This distributes the server's time overhead across more inferences, thereby increasing the overall throughput. However, blindly increasing $\mathbf{F}$ can reduce the flexibility and effectiveness of the cache. To investigate the impact of $\mathbf{F}$ on inference performance, we test the VGG16\_BN model on a dataset containing 50 classes from UCF101. The results are shown in the Fig. \ref{fig:Scale} (b).
% As $\mathbf{F}$ increases, the average inference latency initially decreases sharply and then stabilizes after $\mathbf{F}$ reaches 120. The inference accuracy follows a similar trend. The initial decrease and subsequent stabilization in latency are primarily because the impact on the average inference latency of the server-side time overhead diminishes as $\mathbf{F}$ increases, eventually becoming negligible. The changes in accuracy can be explained as follows. In the test dataset, a single video roughly corresponds to 25 to 70 consecutive frames. As $\mathbf{F}$ increases, the timeliness of the cache decreases, reducing the accuracy of cache hits, which leads to an overall decline in inference accuracy. When $\mathbf{F}$ exceeds 120, COLA struggles to make distinct assessments of the recency for each class effectively, and accuracy stabilizes. After weighing various factors, $\mathbf{F}=60$ is found to be more suitable here, as the accuracy loss from further increasing $\mathbf{F}$ is not offset by the reduction in inference latency. The appropriate $\mathbf{F}$ value is related to the characteristics of the dataset.

% There are various methods available to further enhance the scalability of COLA. For instance, the independent nature of cache allocation for each client allows for parallel processing using multi-threading. Implementing an asynchronous mode can reduce collisions among client requests. Using non-blocking cache requests at the client side (continuing inference while requesting the cache) can prevent server-side time overhead from directly impacting local inference latency. The actual effectiveness of these methods remains to be verified through future research.




==> his/introduction11.tex <==
% I
Deep neural networks (DNNs) have become increasingly prevalent in practical computer vision tasks, such as virtual/augmented reality (VR/AR) \cite{yi2020eagleeye, li2020object} and autonomous driving \cite{kumar2021omnidet, yu2020bdd100k}. 
Traditionally, DNN-based image processing tasks have been managed via cloud servers, but this approach faces some significant challenges.
First, offloading tasks to servers entails substantial data transmission that will adversely affect the Quality of Service (QoS). 
This is particularly problematic in latency-sensitive applications such as autonomous driving, where delays will induce critical consequences. 
Second, there is a growing emphasis on privacy protection, exemplified by regulations such as the General Data Protection Regulation (GDPR) \cite{zaeem2020effect} in the European Union, which is one of the toughest privacy laws worldwide.
These considerations have catalyzed a shift towards edge computing \cite{cao2020overview, zeng2020coedge, shuvo2022efficient}, where inference processes migrate closer to the data sources. 
This paradigm not only mitigates latency issues by reducing dependency on distant cloud servers but also enhances data privacy by localizing data processing.

% II
The enhanced computing capabilities of edge devices have facilitated the proliferation of visual tasks, with driver assistance systems being a prime example.
These tasks impose stringent QoS requirements, such as lower latency and higher throughput.
In automotive video analysis applications, achieving a response latency within 80 milliseconds, along with vehicle recognition accuracy of $\geq$ 95\% and traffic sign recognition accuracy of $\geq$ 92\%, is essential to further enhance the user experience \cite{ogden2021many}.
To achieve these goals, a natural solution is to leverage the caching mechanism \cite{huynh2017deepmon, xu2018deepcache, li2021boosting}, which exploits the high temporal locality of video streams and the similarity between consecutive frames to accelerate inference.
Specifically, this approach stores the results of previous inferences in a cache, allowing for quick access to avoid redundant computations for similar or identical frames in video streams.



% III
Despite the potential, in order to boost inference performance in a multi-client setting, two primary challenges need to be addressed.
(1) \textbf{Feature Dynamism}. 
The video data on the client is highly dynamic, with significant changes in data feature over time and location  \cite{xu2018deepcache, ramesh2019sports}. For example, as day turns into night, the feature of data captured by vehicle-mounted cameras can dynamically change, leading to cached data becoming quickly outdated. 
Suppose the cache management mechanism cannot adapt flexibly to these dynamics, to promptly update or replace stale data, it will result in a decrease in cache utilization and cache hit rates, thereby increasing system overhead and response latency.   
(2) \textbf{Data Imbalance}. 
The data generated by clients exhibits significant non-uniform distribution characteristics, \ie, data imbalance, which is manifested in two aspects.
On the one hand, the heterogeneity of client data, also known as non-independent and identically distributed (non-IID) data, presents a significant challenge. For instance, images captured by multiple cameras participating in a collaborative driving assistant task can be significantly diverse \cite{chiu2020semisupervised}. 
On the other hand, the long-tail distribution of client data adds another layer of complexity. In the context of automobile video analysis, normal driving behaviors occur with relatively high frequency, whereas abnormal behaviors, though infrequent, are varied, thus creating a rich long-tail distribution \cite{zhang2021videolt, perrett2023use}. 
The data imbalance characteristics challenge traditional caching mechanisms, such as the Least Recently Used (LRU) strategy \cite{chrobak1999lru}. They make it difficult to efficiently manage the caching and retrieval of rare event data, harming cache efficiency.




% IV
% 下面两段修改
% 1、要围绕表里的缺点，体现如何解决挑战
% 2、逻辑性
To address the aforementioned challenges, researchers have made significant efforts. 
For instance, LearnedCache \cite{balasubramanian2021accelerating} uses multiple exits and learned models to emulate caching operations, allowing for early inference termination upon cache hit prediction, thus accelerating inference. 
Although LearnedCache can handle feature dynamism through frequent retraining, this approach degrades QoS due to high response latency and low throughput, especially with imbalanced data distributions.
To mitigate this, SMTM \cite{li2021boosting} employs low-dimensional representations (\ie, semantic information) of intermediate inference results as cache-matching entries. This method assesses the importance of different classes to address long-tail distribution challenges and continuously computes new semantic representations to cope with feature dynamism. However, the cache allocation strategy of SMTM often leads to increased lookup time and overall latency when multiple classes frequently appear in inference scenarios. 



The above methods primarily focus on accelerating centralized inference in single-client environments. However, with the development of edge intelligence, collaboration among multiple clients for boosting inference is being actively explored. 
FoggyCache \cite{guo2018foggycache} introduces cross-client approximate computation reuse with caching, emphasizing spatial-temporal correlation among client data. Initially, inference requests are processed locally; upon cache misses, queries are submitted to the server, and local caches are updated using the LRU replacement policy. 
FoggyCache addresses the non-IID issue by aggregating samples from different clients for cloud-side lookup entries, using cross-client data reuse to accelerate inference collectively. 
However, feature dynamism leads to feature shifts that render old records obsolete, wasting memory. In long-tail scenarios, the LRU policy often fails, reducing the cache hit ratio and efficiency.
In summary, existing approaches fail to fully address feature dynamism and data imbalance challenges, as illustrated in Table \ref{table1}.
\begin{table}[t]
	\centering
	\caption{The comparison of the previous schemes and COLA.}\vspace{3mm}
	\label{table1}
	\begin{tabular}{c | c | c | c}
		\hline
            \rule{0pt}{8pt}
    		\multirow{2}{*}{Schemes}   &  Long-Tail         &   non-IID   &  Feature  \\
            \rule{0pt}{8pt}
                     &  Distribution         &   Data   &  Dynamism  \\
		\hline
            \rule{0pt}{12pt}
                LearnedCache \cite{balasubramanian2021accelerating}    &  \ding{53}   & \ding{53}     & \checkmark  \\
            % \hline
            \rule{0pt}{12pt}
                SMTM \cite{li2021boosting}           &  \checkmark  &  \ding{53}    &  \checkmark \\
            % \hline
            \rule{0pt}{12pt}
                FoggyCache \cite{guo2018foggycache}       &  \ding{53}  &  \checkmark    &  \ding{53} \\
            % \hline
            \rule{0pt}{12pt}
                \textbf{COLA} & \checkmark & \checkmark & \checkmark \\
		\hline
	\end{tabular}\vspace{-0.2cm}
\end{table}

% V
To this end, we propose COLA, which leverages a multi-client collaborative caching mechanism, to accelerate inference.  
% 全局聚合更新
Specifically, COLA utilizes a client-server hierarchical caching approach. The server maintains a two-dimensional global cache table, where the columns correspond to the preset cache layers of the model, and the rows correspond to the entries of classes at different layers. 
COLA periodically aggregates information from clients to update the global cache at the server, mitigating the effects of non-IID data and capturing contextual feature changes in the client. 
Additionally, COLA maintains global state information to assist with cache updates and allocations.
% 分配
Then, the server allocates new personalized caches to each client which involves extracting sub-tables corresponding to hot-spot classes at specific cache layers from the global cache. 
% 推理
Upon receiving the cache, clients perform model inference with caching.
During inference, the model sequentially performs cache lookups at each activated cache layer, calculating cumulative scores for each class and checking for cache hits. If a cache hit occurs, the inference process is terminated early, and the cached result is returned.


COLA offers significant advantages over existing cache-based methods. 
Specifically, the hierarchical caching mechanism in COLA effectively addresses feature dynamism and data imbalance among different clients through global cache updates and adaptive client-side cache allocation.
Nevertheless, two key challenges remain for efficient inference with COLA. 
Firstly, the number and location of active cache layers in the model significantly affect the cache lookup cost and effectiveness. Too few cache layers will reduce cache hit rates and acceleration opportunities, while too many layers will increase the average inference latency (see Section \ref{sec:motivation 2}). Thus, \textit{activating the appropriate cache layers in the model (\ie, columns in the global cache) is crucial} for balancing accuracy performance and lookup overhead.
Secondly, we observe that the number of frequently occurring classes may vary a lot under different scenes. In scenarios where a small number of classes frequently appear, using a cache with a fixed large number of classes may dilute the benefits of cache hits due to time wasted on lookups. Conversely, when the number of frequently occurring classes exceeds the number of classes in the cache, it will lead to heavy cache misses or even erroneous hits. Therefore, another challenge is \textit{how to dynamically adjust the number of hot-spot classes in the cache entries (\ie, rows in the global cache)} to improve inference accuracy and reduce inference latency.
The main contributions are summarized as follows:



\begin{itemize}
    \item We propose an efficient framework COLA, which leverages a multi-client collaborative caching mechanism, to enhance inference performance.
    COLA performs global cache updates at the server and dynamically allocates cache entries for each client to handle feature dynamism and imbalanced data distribution. 
    
    \item To address the challenges in COLA, we propose a heuristic greedy cache allocation algorithm to dynamically determine the appropriate cache layers and the number of hot-spot classes in the cache based on the data distribution and the recent local class occurrence patterns of each client. 

    \item We evaluate COLA through extensive experiments. Under a constraint of a 3\% accuracy loss, COLA significantly reduces average inference latency, achieving reductions of 23.01\% to 45.19\% for VGG and ResNet. 
    Additionally, COLA achieves latency reductions of 16.67\%-21.26\% on the ResNet101 model compared to acceleration baselines.
    % Even under the given accuracy loss of 1\%, COLA achieves a reduction in inference latency of over 18.18\% on complex models (\eg, ResNet-101).

    
    % Furthermore, even under higher latency reduction scenarios, COLA exhibits superior performance in terms of accuracy, compared to the existing baselines.
    %This outperforms the baseline methods which achieve latency reductions ranging from 9.2\% to 28.1\%. Furthermore, even under higher latency reduction scenarios, our method exhibits superior performance in terms of accuracy. 
    %These experimental results confirm the effectiveness of our approach.
\end{itemize}



% The organization of this paper is as follows. Section 2 introduces the background and related works of our research. Section 3 shows the motivations in detail. Section 4 presents the workflow of our system. Section 5 describes the formalization of the problem and the proposed algorithm. Section 6 showcases the experimental results and performance analysis. Finally, Section 7 provides a summary of the entire paper.

==> his/motivation8.tex <==
% \subsection{Preliminaries}

% % In this section, we briefly introduce some background knowledge of this paper, such as edge inference, CNN model, and cache-accelerated inference. Then we explain the motivation for using caching and adjusting cache size.

% \subsection{Motivation}
% 1.为什么用cache？
% （1）用图或表描述数据集的时间局部性；
% （2）用图描述数据集具有长尾分布；


% 2.为什么选择cache条目，大小？（把不使用cache用图的一个数据列表示）
% （1）用图描述cache大小与额外计算量（时延）的关系
% （2）用图描述cache大小与命中率（准确性损失）关系
% 以上两种可以描述缓存条目多少（表的行数）带来的影响
% （3）用图表现CNN不同层推理时间
% （4）用图表现CNN推理中不同层缓存退出概率（缓存命中率）
% 以上两种可以描述缓存层数多少（表的列数）带来的影响

% 3.不同客户端帮忙推理
% 对两个客户端应用全局更新，比较有无全局的缓存命中率（或者准确率损失）区别
\subsection{Inference with Caching}

Given the inherent high temporal locality of continuous visual inference, caching is commonly employed to reduce inference latency and enhance long-term throughput for tasks such as VR/AR.
The pioneering work, \eg, DeepMon \cite{huynh2017deepmon}, introduces a caching method that accelerates inference by reusing intermediate computation results from the previous frame in a video stream. Subsequently, works such as DeepCache \cite{xu2018deepcache} have further refined and proposed new caching mechanisms to achieve reuse of similarity over longer time periods.
In this paper, we mainly employ a class-based semantic caching mechanism \cite{li2021boosting}. 
During inference, the model is partitioned into multiple blocks based on preset cache locations, with cache layers set between these blocks.
The cache layers are populated with low-dimensional feature representations of hot-spot classes, resulting in a relatively small overall cache size. 
At any cache layer $j$, each cache entry corresponds to the semantic vector center of a class in the classification task, and the model extracts a one-dimensional semantic vector through global average pooling. 
Then we calculate the cosine similarity between the semantic vector and the cache entry of hot-spot class $i$, denoted as $\mathbf{C}_{i,j}$.
To enhance discriminative robustness, the cross-layer accumulated cosine similarity $\mathbf{A}_{i,j}$ of class $i$ in layer $j$ is used as follows:
\begin{equation}
    \mathbf{A}_{i,j} = \mathbf{C}_{i,j} + \alpha \cdot \mathbf{A}_{i,(j-1)}
\end{equation}
Note that, a decay coefficient $\alpha$ (set to 0.5 in this case) is employed to diminish the weight of previous cache layers. 
Assuming classes $a$ and $b$ have the first and second largest cumulative cosine similarity in cache layer $j$.
The cross-layer accumulated cosine similarities of classes $a$ and $b$ are denoted as $\mathbf{A}_{a,j}$ and $\mathbf{A}_{b,j}$. Then the discriminative score $\mathbf{D}_j$ of the current layer $j$ is calculated as:
\begin{equation}
    \mathbf{D}_j = \frac{ \mathbf{A}_{a,j} - \mathbf{A}_{b,j} }{ \mathbf{A}_{b,j} } 
\end{equation}
The cache hits when the discriminative score $\mathbf{D}_j$ exceeds the predefined threshold $\bm{\Theta}$. In this case, the class $a$ is outputted as the classification result for this iteration and the inference process terminates. If the cache misses, the inference process continues.



\subsection{Motivations for Framework Design}

In this section, we first analyze the impact of cache size on inference latency. 
Then, we explore the influence of the number of cache layers and the number of hot-spot classes on the inference performance, such as hit ratio and accuracy. Finally, we compare the effectiveness of the cache with and without global updates in multi-client settings.


% 图的替换修改 Number of Cache Layers
\begin{figure}[t]
  \centering
  \subfigure[Latency with different cache sizes]{\includegraphics[width=1.66in]{fig/2.2.pdf}}
  \hspace{0.5mm}
  \subfigure[Performance of each cache layer]{\includegraphics[width=1.7in]{fig/2.3.pdf}}
  \caption{The result of ResNet101 on a subset of 50 classes from UCF101. (a) The horizontal axis represents the percentage of the activated cache size relative to the total cache size, with 100\% indicating that the entire cache is activated. (b) Figure shows the hit ratio and accuracy performance of different cache layers.}
  \label{fig:fig_1}
\end{figure}

% \textit{\textbf{1) Different cache sizes exhibit varying effects on inference latency.}}
\textit{\textbf{1) Increasing cache size initially reduces latency, but excessively large caches lead to increased latency.}}
% 这个地方写语义缓存（暂定）
In semantic cache inference, caches can be set after each convolutional layer of the model, allowing for multiple cache layers within the model. For instance, in a ResNet-101 model, up to 34 cache layers can be inserted. These caches have a relatively small size; for the UCF101 task, the total cache size is approximately 3.2 MB, which is 1.95\% of the model size \cite{li2021boosting}. Despite the small memory footprint, the computational overhead for cache lookups is significant. The total lookup latency for all 34 cache layers constitutes 56.22\% of the inference latency without caching.


% 
In order to investigate the impact of cache size on inference performance, we adopt the ResNet-101 model on a subset of 50 classes from the UCF101 dataset with different cache sizes.
% 
The cache size is determined by the number of cache layers and the number of hot-spot classes in the cache. 
% (\ie, the number of entries at each cache layer). 
To mitigate the influence of the cache entry selection algorithm, we set the number of hot-spot classes to the total number of classes. 
% This ensures that each cache layer contains entries for all classes.
% We control the cache size by adjusting the number of cache layers and activating the corresponding cache layers at regular intervals across the 34 layers.
% We use the percentage of total cache size as the horizontal axis for an easy understanding of the relative relationships between different settings.
We control the cache size by adjusting the number of cache layers and activating them at regular intervals across the 34 layers. Using the cache size when all 34 layers are activated (approximately 3.2MB) as a baseline, we use the percentage of this baseline as the horizontal axis for an easy understanding of the relative relationships among different settings.
% 
The average inference latency and accuracy are shown in Fig. \ref{fig:fig_1}(a). 
As the cache size varies, inference accuracy remains stable, with accuracy loss consistently below 2\%. 
Initially, as cache size increases, the average inference latency rapidly decreases, reaching its lowest point when the activated cache size is 10\% of the total cache size. This configuration reduces the average latency by 28\% compared to the setting without caching. As cache size continues to increase, latency gradually rises slightly.
% 
These results indicate that using a cache can effectively reduce average inference latency while incurring low accuracy loss. However, a larger cache size does not necessarily improve performance due to increased lookup times. Therefore, it is crucial to judiciously control cache size to balance lookup overhead and cache hit benefits, achieving optimal performance.


\textit{\textbf{2) Different cache layers and the number of hot-spot classes exhibit varying lookup time, hit ratio, and accuracy.}}
Based on the previous experiments, we conclude that constraining the cache size within a certain threshold is essential for effective latency reduction.
We can adjust the cache size to meet the threshold from two aspects: the number of cache layers and the number of hot-spot classes in the cache.
Model inference with multiple cache layers can increase the overall cache hit ratio, but it results in longer cache lookup times. 
Similarly, increasing the number of hot-spot classes will enhance the likelihood of cache hits but extend lookup times.
To investigate the effect of these two factors in detail, we conduct experiments using the previously described ResNet-101 and dataset.

First, we measure the hit ratio and hit accuracy of different cache layers when all cache layers are activated. 
As shown in Fig. \ref{fig:fig_1}(b), the hit ratio is high in shallow and deep cache layers but low in middle layers. This pattern emerges because easily inferrable samples are hit early. In deeper cache layers, intermediate features become more distinctive, increasing the hit ratio. Middle cache layers naturally have lower hit ratios. Hit accuracy is lower in shallow and deep cache layers. This may be due to insufficient feature discriminability in shallow layers, while deep layers mostly hit difficult samples, resulting in decreased accuracy. 
Shallow cache layers offer higher latency reduction benefits, while deep layers provide better accuracy. 
Therefore, these observations underscore the necessity for careful selection of cache layers to optimize the trade-off between latency reduction and accuracy.


\begin{table}[t]
\centering
\setlength{\abovecaptionskip}{10pt}%
\setlength{\belowcaptionskip}{0pt}%
\footnotesize
\caption{The average inference latency (Late.) and accuracy (Acc.) of ResNet101 with different number of hot-spot classes in the cache on a subset of 50 classes from UCF101 and ImageNet-100 (0 means without cache).}
\label{table2}
\begin{tabular}{ c c c c c}
\hline
\rule{0pt}{8pt}
           Number of & \multicolumn{2}{c}{UCF101} &  \multicolumn{2}{c}{ImageNet-100} \\
\cline{2-5}
\rule{0pt}{8pt}
hot-spot classes  & Late.(ms) & Acc.(\%) & Late.(ms) & Acc.(\%) \\
\hline
\rule{0pt}{8pt}
0   & 40.58 & 80.56  & 40.33  &  82.07   \\
\hline
\rule{0pt}{8pt}
10   & 23.56 & 47.51  & 25.98  & 35.40    \\
\hline
\rule{0pt}{8pt}
30   & 29.23 & 61.45  & 28.70  & 62.81    \\
\hline
\rule{0pt}{8pt}
\textbf{50}   & \textbf{30.53} & \textbf{80.08}  & \textbf{29.08}  & \textbf{81.46}    \\
\hline
\rule{0pt}{8pt}
70   & 33.36 & 80.12  & 33.04  & 81.47    \\
\hline
\rule{0pt}{8pt}
90   & 36.04 & 80.07  & 35.45  & 81.21    \\
\hline
\end{tabular}
\end{table}

% 就两个数据集细化讨论？
Second, we test the effect of the number of hot-spot classes in the cache on the inference performance.
Based on the previous experiment setting, we add ImageNet-100 to enrich our results.
From the test results in Table \ref{table2}, as the number of hot-spot classes increases, both latency and accuracy rise. When the number of hot-spot classes exceeds 50, the accuracy stabilizes, with a loss of less than 1\% compared to the method without caching.
This trend reflects the trade-off between cache hit ratio and lookup latency. Initially, increasing hot-spot classes improves hit ratio and accuracy but also increases lookup time. The optimal balance occurs around 50 classes, after which further expansion yields diminishing returns on hit ratio and accuracy while continuing to increase latency.
In conclusion, it is pivotal to appropriately select cache layers and the number of hot-spot classes for optimizing cache efficiency and ensuring accurate inference results.



\textit{\textbf{3) Global updates exhibit effects on addressing imbalanced data distributions and feature dynamism.}}
% 
In the implemented caching mechanism, the cache entries (\ie, low-dimensional semantic centers) of each class at different cache layers are crucial for cache lookups. Cache hits and inference outcomes depend on the similarity between the intermediate semantic vector of input and cache entries. The accuracy of cache hits relies on the representativeness of cache entries.
% 
However, discrepancies between training data and real client data will reduce the performance of cache entries during inference. Thus, updating global cache entries with client inference data is necessary to improve adaptability. 
Moreover, client data often exhibit non-IID characteristics, such as varying image data from traffic intersections and pet shop cameras. 
% 
Inspired by federated learning, we periodically aggregate semantic vectors from different clients into a global cache table to leverage diverse datasets.
We collect inference samples from clients and use their computed semantic vectors from each cache layer to update the global cache table. 
The global update is performed via weighted summation of new semantic vectors and corresponding existing entries of the same class and layer. This process incorporates diverse semantic information from various clients into the global cache, enhancing its representational power.

\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{fig/pre-aft.pdf}
    \caption{The t-SNE visualization of cosine similarity clustering for the semantic vectors of samples from 4 classes of the UCF101 dataset, cached in the 18-th layer of all 34 cache layers in ResNet101. The larger points represent the cached semantic centers for each class. "Previous" and "After" show the cached entries before and after employing the global updates strategy, respectively.}
    \label{fig:enter-label}
\end{figure}

% % 两张图显示聚类中心的移动
% 这里先用图展示更新后语义中心的移动，再用表显示更新的效果，最后总结
To investigate the effect of global updates on feature dynamism, we select a subset of videos from 20 classes of UCF101 and divide them into day and night categories based on the background. We construct a test dataset with the video sequence first presenting day backgrounds and then transitioning to night backgrounds, aiming to simulate the environmental change from day to night in real scenarios. 
% 更详细的抽样方式？
An equal number of samples are drawn from each class for testing. 
We compare the clustering effects of the cosine similarities between the cached semantic centers and the semantic vectors of samples (from the 18-th layer of all 34 cache layers in ResNet101), with and without global updates. Fig. \ref{fig:enter-label} illustrates the t-SNE 2D visualization of their relative distances. We plot the changing trends of semantic centers for four classes under global updates.  
It can be observed that with global updates, the semantic centers of each class become more closely aligned with their corresponding class sample centers, resulting in improved clustering effects.
% 是否需要一些数据表达，什么数据
The result indicates that the global cache helps align the semantic centers of the cache more closely with the current data characteristics, positively impacting the hit ratio and accuracy of cache lookups during inference.



%Inspired by the above observations, we propose the core mechanism of COLA,  a collaborative caching mechanism that utilizes personalized cache allocation and global aggregation to boost the effect of cache on accelerating inference. 


